Social contagion and asset prices: Reddit's self-organised bull runs

Can unstructured text data from social media help explain the drivers of large asset price fluctuations? This paper investigates how social forces affect asset prices, by using machine learning tools to extract beliefs and positions of `hype' traders active on Reddit's WallStreetBets (WSB) forum. Our stylized model shows that peer effects help explain return predictability and reversals, as well as bubble dynamics. We empirically document that sentiments expressed by WSB users about assets' future performances (bullish or bearish) are in part due to sentiments of their peers and past asset returns. The paper directly estimates the effect of WSB activity on asset prices. We document: that retail trader demand follows WSB discussions through using Trade and Quote (TAQ) data, the predictability of prices from retail trader discourse, the amplified market impact of idiosyncratic investor sentiment from viral content online, and the greater exposure of hype investors to bubbles in the markets.

==> Appendices/Chaotic_prices.tex <==
    \subsubsection{Results -- Chaotic Prices from Coordinated Strategies} 
    \label{app:chaotic_prices}
    
    We evaluate consider the implications of `coordination' and `consensus' among hype investors in two different ways. First, we theoretically determine the sensitivity of price to its various components in Eq. \ref{eq:full_price_dynamic_explained}. We subsequently perform a discrete time simulation, using parameters from the WSB forum found in section \ref{sec:social_dynamics}, to determine the price dynamics one could expect, given the current state of discussions among investors on social media. 
        
    \paragraph{Impact of $\Dot{\chi}$, $\varepsilon_{\chi}$ on Price Stability} Our original derivations offer some insight into the primary components that impact price, as explained after Eq. \ref{eq:full_price_dynamic_explained}. The influence of certain variables appears trivial to evaluate: for example, as $N$ or $M$ in Eq. \ref{eq:full_price_dynamic_explained} increase, social contagion will have greater market impact, consistently with \cite{de1990noise} who find that the fewer `sophisticated investors' there are relative to the `noise traders', the larger is the impact of noise. However, the relevance of $\Dot{\chi}$, detailed in Eq. \ref{eq:dot_phi}, and $\varepsilon_{\chi}$, detailed in Eq. \ref{eq:var_epsilon} (Appendix \ref{app:model}), is less obvious. 
          
    We turn to \cite{hommes2013behavioral} for an understanding of price stability, or instability. We consider a scenario when hype investors begin to discuss a stock but no price impact has been felt (setting $\Dot{p}/p=0$) and analyse the price dynamics that ensue. This system produces a stable steady state at $\phi = 0$ if $\hat{\alpha}/(2\hat{\theta}) \leq 1$, implying that investors are not connected enough for sentiments to amplify. In this scenario, a small value for $\hat{\alpha}/(2\hat{\theta})$ implies that consensus is difficult to reach. However, with $\hat{\alpha}/(2\hat{\theta}) >1$, we arrive at a `pitchfork' bifurcation, as described in \cite{hommes2013behavioral}. The buying intensity produces two stable steady states, $\chi^+ > 0$, $\chi^- < 0$, and one unstable steady state at $\chi^0 = 0$. These interesting dynamics illustrate the potentially important effect of strong feedback, as investors coordinate to buy or sell the asset together.
    
  

==> Appendices/Model.tex <==

\subsection{Validity of model assumptions and aggregating sentiments}
\label{app:model}

    \paragraph{Aggregating sentiments}
    %In this section, we describe how investors reach a buy/sell decision about an asset on aggregate. First, we consider that they form a sentiment $\phi_i$ about an asset based on the signals we consider in Section \ref{sec:social_dynamics}. Their choice to buy / sell the asset is modelled as a quantal response function. The precise steps are outlined here.  
    
    In Section \ref{sec:social_dynamics}, we model the log-odds of investor sentiment $\phi_i$ by a standard multivariate logistic function. This stems from a utility ranking between adopting a positive ($\phi_i = +1$) or negative ($\phi_i = -1$) position on the asset, as a function of observed returns and peer sentiment:
    \begin{align*}
        U(\phi_{i,t+1} = +1) = \epsilon_i^+ + \alpha{\phi}_{t} +\beta r_t - \gamma r_t^2, \quad 
        U(\phi_{i,t+1} = -1) =  \epsilon_i^- - \alpha{\phi}_{t} - \beta r_t - \gamma r_t^2.
    \end{align*}
    An assumption on the distribution of the idiosyncratic terms $\epsilon_i^+$ and $\epsilon_i^-$, which we state in Assumption \ref{assumption:extreme_value}, allows us to derive an expression for the probability of bullish versus bearish sentiment. We write the probability of bullish sentiment as
    \begin{align}
        \text{P}[U(+1) > U(-1)] &= \text{P}(\epsilon_i^+ + \alpha{\phi}_{t} +\beta r_t - \gamma r_t^2 > \epsilon_i^- - \alpha{\phi}_{t} - \beta r_t - \gamma r_t^2), \\
        &= \text{P}(\epsilon_i^- < \epsilon_i^+ + 2 \alpha{\phi}_{t} + 2 \beta r_t), \\ 
        &= \int_{-\infty}^{+\infty} \text{P}(\epsilon_i^- < \epsilon_i^+ + 2 \alpha{\phi}_{t} + 2 \beta r_t | \epsilon_i^+) \times p(\epsilon_i^+) d\epsilon_i^+, \\
        &= \int_{-\infty}^{+\infty} \text{exp}\left[ -\text{exp}\left(- \frac{\epsilon_i^+ + 2\alpha{\phi}_{t} + 2\beta r_t}{2\lambda} \right) \right] \times \frac{1}{2\lambda}\text{exp}\left[ - \frac{\epsilon_i^+}{2\lambda} -\text{exp}\left(- \frac{\epsilon_i^+}{2\lambda} \right)  \right] d\epsilon_i^+, \label{eq:probability_density_assumption} \\
        &= \frac{\text{exp}\left(\frac{\alpha{\phi}_{t} + \beta r_t}{\lambda}\right)}{\text{exp}\left( \frac{\alpha{\phi}_{t} + \beta r_t}{\lambda}\right) + 1},
    \end{align}
    where step \ref{eq:probability_density_assumption} follows from the fact that we are integrating the cumulative density of $\epsilon_i^-$, with scale $2\lambda$, over the support of $\epsilon_i^+$, with marginal density with marginal density $p(\epsilon) = \text{exp}[-\epsilon/2\lambda -\text{exp}(-\epsilon/2\lambda)]/2\lambda$. The final simplification comes from the fact that $U(\phi_{i,t+1} = +1)$ and $U(\phi_{i,t+1} = -1)$ are symmetric in parameters $\alpha, \beta$ and $\gamma$. If we want to keep them distinct, we arrive at the quantal response function for the probability of positive or negative sentiment:
    \begin{align*}
          \phi_{i,t+1}^D =
          \begin{cases}
          +1, & \text{with probability} \frac{\text{exp}\left[(\alpha{\phi}_{t} +\beta r_t - \gamma r_t^2)/2\lambda\right]}{\text{exp}\left[( \alpha{\phi}_{t} + \beta r_t - \gamma r_t^2)/2\lambda\right] + \text{exp}\left[( -\alpha{\phi}_{t} - \beta r_t - \gamma r_t^2)/2\lambda\right]}, \\
          -1, & \text{with probability } \frac{\text{exp}\left[( -\alpha{\phi}_{t} - \beta r_t - \gamma r_t^2)/2\lambda\right]}{\text{exp}\left[( \alpha{\phi}_{t} + \beta r_t - \gamma r_t^2)/2\lambda\right] + \text{exp}\left[(-\alpha{\phi}_{t} - \beta r_t - \gamma r_t^2)/2\lambda\right]}.
          \end{cases}
    \end{align*}
    Therefore, we can model the aggregate buying intensity by summing $\phi_{i,t+1}^D$ across the $N$ hype investors, which yields the well-known hyperbolic tangent function: 
    \begin{align*}
        \phi_{t+1} = \text{tanh}\left[ (\beta r_t + \alpha \phi_{t})/\lambda \right].
    \end{align*}
    Our Online Appendix includes additional details on the properties of this function.
    % \begin{figure}[ht]
    %     \begin{center}
    %      \includegraphics[width=0.5\linewidth]{Figures/Simulation/errors.pdf}
    %      \caption{\textbf{Distribution of $\epsilon_i$}; We plot the observed distribution of residuals from the regressions presented in Eq. \ref{eq:epsilon_i}, which we use to estimate author's $\epsilon_i$. We overlay our histogram of observations with a fitted type-I error distribution Probability Density Function (PDF). The location parameter for our fitted type-I EV is $-1.22$ and the scale parameter is $2.08$}
    %      \label{fig:dist_epsilons}
    %     \end{center}
    % \end{figure}    

    
    \paragraph{Validity of Assumption \ref{assumption:other_investors}}  \citet{shiller1984stock} demonstrates that fully `rational investors' (a category of investor we liken to non-hype investors in this paper) would anticipate persistent shifts in hype investors' demand for a stock, potentially justifying their willingness to pay a price different from that derived by discounting a stream of dividends. Our assumption is, therefore, somewhat reasonable as it implies that non-social investors hold the asset at every price point, and simply trade to keep their exposure constant. 
    
    \paragraph{Validity and implications of Assumption \ref{assumption:capacity}} We consider a shift in the number of hype investors $N$ to be exogenous for the purposes of this section. We also hold the ratio $M/p_t$ constant: this implies that the balances hype investor have invested in the asset, $M$, increase and decrease proportionally with the asset's price. Any changes in price are met with proportional profits / decreases in capital $M$ -- potentially due to gains from investments or moving capital elsewhere, allowing us to keep the ratio $M/p_t$ fixed.
    
    % \paragraph{Contagion} We leverage our findings from Section \ref{subsec:contagion} to understand the dynamics which govern how hype investors enter the market for a certain asset through word-of-mouth information transmission. Ignoring the presence of alternative investment options, the mechanism for information transmission is alone responsible for the spread of awareness on the asset as an investment possibility (unlike the empirical framework, which assumed users to make a choice over many alternative investment options). We categorise the fixed number of hype investors $N$ between the shares that are i) unaware ($z$), ii) aware ($a = A/N$), and iii) aware but disinvested ($n$):
    % \begin{align*}
    %     \dot{z} = -c a z, \quad
    %     \dot{a} = c az - d a, \quad
    %     \dot{n} = d a, \quad
    %     z + a + n = 1.
    % \end{align*}
    % As in Section \ref{subsec:contagion}, parameter $c$ is the average rate at which awareness of an investment opportunity transmits between investors per contact case, assuming homogeneous mixing, and $d$ is the rate at which trading on a stock by an investor ceases permanently. While WSB only reflects awareness over time alone, and not the presence of unaware or disinvested users, we can still use time series data on the count of authors discussing specific stocks to estimate a logistic model for coefficients $c$ and $d$, as in Section \ref{subsec:contagion}. 
    
    % \paragraph{Derivation of  Eq. \ref{eq:aggregate_buying_intensity}}
    % We use our utility framework and empirical results from section \ref{sec:consensus_results} to propose that individual investors update their sentiments about assets according to Eq. \ref{eq:consensus_model}:
    % \begin{align*}
    %     \phi_{i,t} = \kappa\phi_{i,(t-1)} + \alpha \Bar{\phi}_{-i,(t-1)} + \beta r_{t} + \gamma \sigma(r_{t}) + \epsilon_{i,t}.
    % \end{align*}
    % We propose that function $f$ is a quantal response function:
    % \begin{align}
    % \label{eq:opinion_logit}
    %       f(\phi_{i,t})=
    %       \begin{cases}
    %       +1, & \text{with probability }\ e^{\lambda\phi_{i,t}}/(e^{\lambda\phi_{i,t}}+1) \\
    %       -1, & \text{with probability } 1/(e^{\lambda\phi_{i,t}}+1),
    %       \end{cases}
    % \end{align}
    % with $\phi_{i,t}$ defined as before, $\lambda$ specifying the amount of noise in the decision process (with further discussions on $\lambda$ available in \citealt{bouchaud2013crises}). 
    
    % \textit{Aggregate Buying Intensity}
    % Given a definition for $\phi_{i,t}$, we can derive the aggregate buying intensity, $\phi(t,p)$, between all hype investors that are active in an asset at a given point in time. Since we are interested in the overall impact that hype investors have on price, deriving a cumulative consensus dynamic is of particular interest. 
    
    % The formulation of individual $\phi_{i,t}$, as in Eq. \ref{eq:opinion_logit}, yields the following functional form for $\phi(t,p)$, computed as the average buy/sell decision across all active investors:
    % \begin{align}
    %     \phi(t,p) = \frac{e^{\lambda\Bar{\phi}_t} -1 }{e^{\lambda\Bar{\phi}_t}+1} = \text{tanh} \left( \frac{\lambda \Bar{\phi}_t}{2}\right),
    % \end{align}
    % where the first equality stems from the fact that we are taking an average across identical Bernoulli random variables; $\Bar{\phi}_t$ is an estimate of the population average.
    
    % We substitute $\beta$ and $\gamma$ as our estimates. Individual buy/sell decisions are derived from the sentiments expressed by neighbors and aggregated by a single individual. For simplicity, we equally weight an author's prior opinion and that of his neighbours. The aggregate buying intensity can then be computed as:
    %     \begin{align}
    %         \phi(t,p) &= \text{tanh}\left[ \frac{\lambda}{2} \left( \hat{\beta}  \frac{\Dot{p}}{p} - \hat{\gamma} \left(\frac{\Dot{p}}{p}\right)^2 + \hat{\alpha} \Bar{\phi}_{(t-1)} \right) \right].
    %     \end{align}
    
    % \paragraph{Derivation of Eq. \ref{eq:full_price_dynamic_explained}}
    % In this section, we show the steps for deriving Eq. \ref{eq:full_price_dynamic_explained}. We begin with: 
    %     \begin{align*}
    %              \frac{\Dot{p}}{p} = \frac{MN}{pQ} \times \frac{d}{dt}[a(t) \phi(p,t)].
    %     \end{align*}
    %     The derivative with respect to time is
    %     \begin{align*}
    %             \frac{\Dot{p}}{p} = \frac{MN}{pQ} \left( \frac{da}{dt} \phi + \left[ \frac{\partial \phi}{\partial t} + \frac{\partial \phi}{\partial p} \frac{dp}{dt} \right]a \right),
    %     \end{align*}
    %     where we take the partial derivative of $A$, and break down the derivative of $\phi$ with respect to time and price, since both determine the overall change in $\phi$. Rearranging yields 
    %     \begin{align*}
    %             \frac{\Dot{p}}{p} - \frac{MNa}{pQ} \left( \frac{\partial \phi}{\partial p} \frac{dp}{dt}\right) = \frac{MN}{pQ} \left( \phi \frac{da}{dt}  + a \frac{\partial \phi}{\partial t} \right),
    %     \end{align*}
    %     and the left-hand side is simplified as
    %     \begin{align}
    %             \frac{\Dot{p}}{p} \left(1 - \frac{MNa}{Q} \left( \frac{\partial \phi}{\partial p}\right) \right) = \frac{MN}{pQ} \left( \phi \frac{da}{dt}  + a \frac{\partial \phi}{\partial t} \right),
    %             \label{eq:intermediate_eq1}
    %     \end{align}
    %     given $\Dot{p} = dp/dt$. %Substituting $dA/dt = cAV -rA$ into the right hand side yields
    %     %\begin{align*}
    %     %        \frac{\Dot{p}}{p} \left(1 - \frac{MNa}{Q} \left( \frac{\partial \phi}{\partial p}\right) \right) = \frac{M}{pQ} \left( \chi [cAV-rA]  + A \frac{\partial \phi}{\partial t} \right).
    %     %\end{align*}
    %     %Factoring $A$ on the right-hand side of the equation and noting $\Dot{\phi} = \partial \phi/\partial t$ yields
    %     %\begin{align}
    %     %\label{eq:intermediate_eq1}
    %     %        \frac{\Dot{p}}{p} \left(1 - \frac{MA}{Q} \left( \frac{\partial \phi}{\partial p}\right) \right) = \frac{MA}{pQ} \left( \phi [cV-r]  + \Dot{\phi} \right).
    %     %\end{align}
    %     which gives us the components (1) and (3) on the right hand side of our equation. 
        
    %     To derive component (2), recall that
    %     \begin{align*}
    %         pQ = pY+pS,
    %     \end{align*}
    %     and denote $s = S/Q$, the proportion of shares owned by non-hype investors. Finally, the hype investor asset demand identity holds, $pY = \phi M N a$, such that the total value of shares owned by hype investors ($pY$) equals the number of active hype investors in the market, $Na$, the average amount of money they hold, $M$, and their buying intensity $\phi$. Thus, we rearrange the identity
    %     \begin{align*}
    %         pQ &= pY+pS, \\
    %         1 &= \frac{\phi M A}{pQ} + s, \\
    %         (1-s) &= \frac{\phi M Na}{pQ}.
    %     \end{align*}
    %     We define the price elasticity of buying intensity as
    %     \begin{align*}
    %         \varepsilon_\phi = -\frac{p}{\phi} \frac{\partial \phi}{\partial p},
    %     \end{align*}
    %     such that
    %     \begin{align*}
    %         (1-s)\varepsilon_\phi &= -\frac{\phi M Na}{pQ}\times \frac{p}{\phi} \frac{\partial \phi}{\partial p} \\
    %         &= -\frac{ M Na}{Q} \frac{\partial \phi}{\partial p}.
    %     \end{align*}
    %     Substituting this results into Eq. \ref{eq:intermediate_eq1} yields
    %     \begin{align*}
    %         \frac{\Dot{p}}{p} \left(1+(1-s)\varepsilon_\phi \right) = \frac{MN}{pQ} \left( \phi \dot{a}  + \dot{\phi} a \right).
    %     \end{align*}
    %     Eq. \ref{eq:full_price_dynamic_explained} is obtained by dividing by the elasticity term:
    %     \begin{align*}
    %         \frac{\Dot{p}}{p} = \frac{MN}{pQ} \times \frac{\phi \dot{a}  + \dot{\phi} a}{1+(1-s)\varepsilon_\phi},
    %         \end{align*}
    %     where
    %     \begin{align}
    %         \Dot{\phi} = \frac{\partial \phi}{\partial t} = \frac{\hat{\alpha}}{2 \hat{\gamma} \left(\frac{\dot{p}}{p}\right)^2 }\text{ sech}^2\left[ \frac{\hat{\beta}  \frac{\Dot{p}}{p} + \hat{\alpha} \phi(p,t)}{2\hat{\gamma} \left(\frac{\Dot{p}}{p}\right)^2} \right]
    %     \label{eq:dot_phi}
    %     \end{align}
    %     %\begin{align}
    %     %    \Dot{\phi} = \frac{\partial \phi}{\partial t} = \frac{\lambda\hat{\alpha}}{2} \text{ sech}^2\left[ \frac{\lambda}{2} \left( (\hat{a} - \hat{a}') \frac{\Dot{p}}{p} - \hat{b} \left(\frac{\Dot{p}}{p}\right)^2 + \hat{\alpha} \phi \right) \right]
    %     %\label{eq:dot_phi}
    %     %\end{align}
    %     is the partial rate of change in buying intensity with respect to time,
    %     \begin{align}
    %          \varepsilon_\phi = -\frac{p}{\phi} \frac{\partial \phi}{\partial p}  = 0
    %     \label{eq:var_epsilon}
    %     \end{align}
    %     is the price elasticity of the buying intensity, and $s = S/Q$ is the fraction of shares owned by non-hype investors. We observe that in our definition of $\phi(p,t)$ depends on returns and investor sentiments, however, does not depend on actual price level, $p$. In other words, investors care about the opinions of others and the change in asset prices, but not in the initial price levels of different assets. Therefore, $\varepsilon_{\phi}$ is zero for our formulation of $\phi$.
        
        %\begin{align}
        %     \varepsilon_\phi = -\frac{p}{\phi} \frac{\partial \phi}{\partial p} = \frac{p\lambda}{2\phi}\left( (\hat{a} - \hat{a}') - \hat{b} \frac{\Dot{p}}{p} \right) \text{ sech}^2\left[ \frac{\lambda}{2} \left( (\hat{a} - \hat{a}') \frac{\Dot{p}}{p} - \hat{b} \left(\frac{\Dot{p}}{p}\right)^2 + \hat{\alpha} \phi \right) \right]
        %\label{eq:var_epsilon}
        %\end{align} 
        
        
%%%%%%% OLD %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %\paragraph{Longer Time Scales and Elasticities of Demand}
    %On longer scales, larger bull runs form, depending on the responsiveness of hype and other investors to price changes. To see this, we write $Y(p)$, the demand function for hype investors, and $S(p)$ for other investors. This time, we assume
    %\begin{align*}
    %    \frac{\partial S(p)}{\partial t} = 0,
    %\end{align*}
    %so that the adjustment in shares held by other investors is purely endogenous with respect to price. The total derivative of Eq. \ref{eq:full_price_dynamic_explained} thus yields
    %\begin{align}
    %\label{eq:law_of_motion_price}
    %    \frac{\Dot{p}}{p} = \frac{1-m}{\left(\varepsilon_Y + s[\varepsilon_S - \varepsilon_Y] \right)} \frac{\Dot{Y}}{Y},
    %\end{align}
    %where 
    %\begin{align*}
    %    \varepsilon_Y = - \frac{p}{Y} \frac{\partial Y(p)}{\partial p}
    %\end{align*}
    %is the price elasticity of demand for hype investors, and, likewise,
    %\begin{align*}
    %    \varepsilon_S = - \frac{p}{S} \frac{\partial S(p)}{\partial p}
    %\end{align*}
    %is the price elasticity of demand for non-hype investors. We denote $s3 = S/Q$, the ratio of shares owned by non-hype investors. Eq. \ref{eq:law_of_motion_price} demonstrates that prices may shoot off indefinitely if, between all investors, increasing prices fail to trigger enough shareholders to sell. A crash would only take place once enough investors decide to increase their response to higher prices, causing a sign reversal in Eq. \ref{eq:law_of_motion_price}. This type of model, where the responsiveness of agents' demand to price varies, is studied extensively by \citet{hommes2013behavioral}, and so we do not dwell on it here.
    
    %\paragraph{Herding and Investor Clusters}
    %This papers offers a deeper exposition of asset demand by hype investors by introducing the effect of consensus among hype investors, and its consequences on price stability. To that end, the particular appeal of social dynamics is in producing movements large enough to overcome the market depth bottleneck. To see this, consider the breakdown of individual investors $i$, which we replicate from \citet{bouchaud2003theory}:
    %\begin{align*}
    %    K = \sum_i \chi_{i}, 
    %\end{align*}
    %where $K$ replaces $Y$ as total demand, to reflect individual demand $\chi_i$ taking values $-1$ should $i$ sell, $0$ if they are neutral, and $+1$ if they buy. There is an implicit assumption that all investors $i$ have the same purchasing power, which we will denote $M$. From Eq \ref{eq:dynamical_price}, it is obvious that individual hype investors, controlling an infinitesimally small fraction of the supply $Y$, are unable to translate their trades into large price movements. However, should investors be linked, such that they coordinate their demand simultaneously, then
    %\begin{align*}
    %    K = \sum_C L(C) \phi_{C}, 
    %\end{align*}
    %whereby hype investors are organised into $C$ clusters of size $L(C)$, trading in direction $\phi_C$. We use $\chi_i$ to denote individual buy/sell decision after the applying the quantal function; $\phi_C$ denotes the aggregate intensity in cluster $C$. This is where our simplifying assumption is useful: heterogeneity in investor size implies that certain clusters emerge from large investors, confusing the effect of consensus by which many small investors $i$ can form an equally-sized cluster. Therefore, this formulation highlights social dynamics, i.e. interactions \textit{between} individuals, as the mechanism for hype investors to drive market fluctuations. 

==> Appendices/Model_stability_analysis.tex <==


%In this section of the appendix, we discuss the methodology behind Section \ref{subsec:stability_analysis}. We precisely outline the steps taken to find our system steady states, as well as show the expected system behaviour around the steady states. 
\subsection{Stability Analysis}
\label{app:stability_analysis}

As mentioned in Section \ref{subsec:stability_analysis}, $r_t$ must be zero at the steady state. This means that steady states of the dynamic system in Eqs. \ref{eq:consensus_model_discrete_1}-\ref{eq:consensus_model_discrete_2} are those for which $\phi_t$ is a solution to Eq. \ref{eq:consensus_model_discrete_1}. Due to the properties of the hyperbolic tangent function (explored thoroughly in the Online Appendix), zero is a unique steady state when $\alpha/\lambda <1$, and two further steady states emerge when $\alpha/\lambda > 1$. Those two additional steady states are solved numerically in all simulation exercises, using a solving algorithm.

The behaviour of our system depends not only on the existence of steady states, but also on the types of steady states that we observe in different stability regions. In a discrete time system, the type of stability around a steady state is dependent on the eigenvalues of the Jacobian matrix at the steady state. The Jacobian matrices at the different steady states are %Table \ref{tab:jacobian_steady_states} shows some types of common behaviours around a single steady state, as they relate to the Jacobian eigenvalues. When a system has multiple eigenvalues, different behaviours can emerge. For example, if we consider two eigenvalues $x_1$ and $x_2$ and $|x_1| > 1$ while $x_2 <1$, we would observe a saddle. Various resources exist to review system steady states, largely originating from the study of physical systems, with \cite{hommes2013behavioral} providing a relevant review for the economic setting.

%\input{Tables/Jacobian_SS}

\begin{align}
    J(0,0) =    \begin{bmatrix} 
            	\alpha & \beta \\
            	C(\alpha - 1) & C\beta
            	\end{bmatrix}, \quad
    J(\phi,0) = \begin{bmatrix} 
            	\alpha \text{sech}^2(\alpha\phi) & \beta \text{sech}^2(\alpha\phi) \\
            	C\left(\alpha\text{sech}^2(\alpha\phi) - 1\right) & C\beta \text{sech}^2(\alpha\phi)
            	\end{bmatrix},
\end{align}
where $\phi \in \{\phi^+, \phi^-\}$. The corresponding eigenvalues for steady state $(0,0)$ are
\begin{align}
\label{eq:eigenvalue_0_0}
    x_1 = \frac{1}{2} \left( C\beta + \alpha + \sqrt{(C\beta + \alpha)^2 - 4C\beta} \right), \quad
    x_2 = \frac{1}{2} \left( C\beta + \alpha - \sqrt{(C\beta + \alpha)^2 - 4C\beta} \right),
\end{align}
and those for steady states $(\phi,0)$ are
\begin{align}
\label{eq:eigenvalue_phi_0_plus}
    x_1 = \frac{\text{sech}^2(\alpha\phi)}{2} \left((C\beta + \alpha) + \sqrt{\text{sech}^2(\alpha\phi)(C\beta + \alpha)^2 - 4C\beta} \right), \\
    x_2 = \frac{\text{sech}^2(\alpha\phi)}{2} \left((C\beta + \alpha) - \sqrt{\text{sech}^2(\alpha\phi)(C\beta + \alpha)^2 - 4C\beta} \right). \label{eq:eigenvalue_phi_0_minus}
\end{align}
These expressions trace different regions of stability as a function of $C\beta$ and $\alpha$ in Figure \ref{fig:stability_regions}. 

Figure \ref{fig:stability_regions} is drawn by solving numerically for the points $C\beta$ for which the eigenvalues in Eq. \ref{eq:eigenvalue_0_0}, on the left, and Eqs. \ref{eq:eigenvalue_phi_0_plus}-\ref{eq:eigenvalue_phi_0_minus}, on the right, switch between the different stability regions. Specifically, we solve for when the complex part of the eigenvalues is equal to zero, and the eigenvalues are on the unit circle. These points are computed by taking a range of values for $\alpha$, then applying a solving algorithm. The solutions are used to distinguish the different regions of stability in Figure \ref{fig:stability_regions}. 

==> Appendices/Sentiment_variabletex <==
\subsection{Sentiment variable creation}
\label{app:sentiment_variable}
We begin with the output of our sentiment classifier, detailed in Appendix \ref{app:bert}. It assigns three probability scores to each submission about a ticker: the probability of a submission being bullish, $P(\phi = +1)$, bearish, $P(\phi = -1)$, neutral, $P(\phi = 0)$. The probabilities sum to one. At the time $t$ when an author $i$ posts about asset $j$, we use the probability scores above to calculate a continuous sentiment score between $(-\infty, \infty)$:
\begin{align*}
\Phi_{i,j,t} = \frac{1}{2} \log \left( \frac{\text{P}(\phi_{i,j,t} = +1)}{\text{P}(\phi_{i,j,t} = -1)} \right).
\end{align*}
Submissions labeled as bullish ($\text{P}(\phi = +1) = 1$), or bearish ($\text{P}(\phi = +1) = 1$), are set to $\text{P}(\phi = +1) = 0.98$, or $\text{P}(\phi = -1) = 0.98$, to retrieve a finite value for the log-odds.

==> Appendices/Simulation.tex <==
% \newpage

\subsection{Asset Price Simulation}
\label{app:simulation}
    
    
    
    %\paragraph{Dynamical System}
    %The key pattern of interest is the effect of a transitory increase in demand, driven by hype, on the price of an asset. To this end, we simulate the following dynamical system:
    %    \begin{align*}
    %        A_{t+1} &= \text{max}\left[ A_t + cV_tA_t - rA_t, A_0 \right], \\
    %        V_{t+1} &= V_t - cV_tA_t, \\
    %        B_{t+1} &= B_0 + (V_0-V_{t+1}) + (A_0-A_{t+1}) \\ 
    %        \phi_{t+1} &= \frac{A_0}{A_{t+1}}\phi_0 + \frac{A_{t+1}-A_0}{A_{t+1}} \text{ tanh}\left[ \frac{\lambda}{2} \left( a \left(\frac{p_t - p_{t-1}}{p_{t-1}}\right) - b \left(\frac{p_t - p_{t-1}}{p_{t-1}}\right)^2 + \alpha \phi_t \right) \right], \\
    %        S_{t+1} &= Q - MA_{t+1}\phi_{t+1}, \\
    %        p_{t+1} &= \frac{p_0S_0}{S_{t+1}},
    %    \end{align*}
    %where a subscript 0 denotes the starting value.
    
    %\paragraph{Parameter Estimation} We choose initialization parameters for our model simulation which are closely related to empirical observations, where this is possible. Values for the price trend, $a$, and aversion to volatility, $b$, are set to an average of the coefficients in the second model of Table \ref{tab:consensus_full_reg} ($a = 0.18$, $b = 0.92$). We arbitrarily set $\lambda$ to $0.9$. The remaining values were set to produce an equilibrium price of 1, and an equilibrium fraction of shares held by non-hype investors of 0.7: initial susceptible investors $V_0 = 200,000$, initial active investors $A_0 = 30,000$, initial recovered investors $B_0 = 0$, contagion rate $c = 5 \times 10^{-7}$, and recovery rate $r = 0.01$. The pattern of contagion produced is displayed in Figure \ref{fig:contagion_plot}. At its peak, over 150,000 hype investors actively buy, or sell, the asset, before returning to the initial value after 225 time steps. For the price dynamics, the remaining inputs are for hype investor capital, $M = 100$, and number of shares, $Q = 1,000,000$. 

    \paragraph{Discrete Time Simulation} We perform a discrete time simulation of our final model, presented in Eq. \ref{eq:full_price_dynamic_explained}.
        
    The choices made to simulate the model include: i) some fixed fraction of hype investors, $a_0$, are always present with a fixed buying intensity, and ii) non-hype investors fix the nominal value of their investment. In practice this implies that hype investors enter the market to buy the asset (since $\phi_0>0$), which other investors sell to them at a higher price. The price changes and coordination of buying strategies affect the intensity with which hype investors purchase the asset in subsequent periods. Gradually, they leave the market until only the starting amount $a_0$ remain, and the price returns to its `true' value.
        
        \begin{figure}[ht!]
            \begin{subfigure}{0.5\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/Simulation/Contagion_plot.pdf}
                \caption{Contagion among Hype Investors} 
                \label{fig:contagion_plot}
            \end{subfigure}
            \hfill
            \begin{subfigure}{0.5\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/Simulation/Price_plot_0.9_0.1and7_0.18_0.92.pdf}
                \caption{Impact on Price} 
                \label{fig:price_plot_baseline}
            \end{subfigure}
            \bigskip
            \begin{subfigure}{0.5\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/Simulation/Price_plot_MU.pdf}
                \caption{MU Observed and Simulated Price Dynamics} 
                \label{fig:contagion_MU}
            \end{subfigure}
            \hfill
            \begin{subfigure}{0.5\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/Simulation/Price_plot_TSLA.pdf}
                \caption{TSLA Observed and Simulated Price Dynamics} 
                \label{fig:contagion_TSLA}
            \end{subfigure}
            \caption{\textbf{Price Impact of Contagion and Opinion Dynamics}; In Figures \ref{fig:contagion_plot}, \ref{fig:price_plot_baseline} we illustrate the hypothetical dynamics that can emerge within our model. On the left, the number of active hype investors in an asset increases steeply until time step 50, after which the number slowly declines to its initial value (as `active' investors `recover'). On the right, at price first increases until time step 50, after which it experiences a volatile crash when consensus formation is strong ($\alpha = 0.7$), then returns to its initial level. In contrast, when consensus formation is weak ($\alpha = 0.1$), very little price impact is observed. Other parameter choices are discussed in Appendix \ref{app:simulation}. Figure \ref{fig:contagion_MU}, \ref{fig:contagion_TSLA} show the dynamics simulated using parameters derived from WSB in the two stocks at a time when the tickers were increasing in popularity within the forum. The stock price displayed is the average weekly close price for each stock (ensuring consistent time steps between asset price and simulation).}
            \label{fig:price_baseline}
        \end{figure}
        
        Since the focus is on asset demand by hype investors, we simulate various parameters for coordination, $\alpha$. Given the complex dynamics, qualitatively different patterns could be generated depending on the choice of demand parameters. The result, in Figure \ref{fig:price_plot_baseline}, displays three important characteristics for scenarios where consensus is strong ($\alpha = 0.7)$ and weak ($\alpha = 0.1)$; other parameters are chosen in line with empirical observations and discussed further below. Under strong consensus, the initial increase in demand, until time step 50, gradually drives up price. Once this growth is depleted, the price crashes dramatically, and extreme volatility persists until time step 150. At this stage, some active investors still remain in the market, but the price follows a steady downward trend until it reaches its initial level. In contrast, the effect under weak consensus is relatively mute, as new entrants fail to adopt the sentiments of existing investors.
        These findings support the conclusions in \cite{de1990noise}, stating that if `sophisticated investors' time horizons are long, compared to `noise traders', they can `buy low, confident that they will be able to sell high when prices revert to the mean'. Eventually, the asset's price reverses to its original level as hype investors exit the market and other investors trade to revert the asset to its fundamental value. 
        
        Figures \ref{fig:contagion_MU}, \ref{fig:contagion_TSLA} on the other hand consider the dynamics that our model implies for two popular stocks within the WSB forum. We initiate the model with coordination and contagion parameters from our data. We emphasize that our goal is not to show that our model can predict stock price movements, but rather that stock price fluctuations, indeed, appear to follow a bursty pattern, consistent with our model and contagion / consensus among hype investors. We observe that in our TSLA simulation, we significantly under-predict the price change. This may be due to our under-estimation of of the number of hype-investors versus other investors, or the fact that following a significant price increase, other investors also change their dynamics. 

    %\paragraph{Simulation Sensitivity} The social dynamics model can reproduce a diverse set of patterns. In this section, we consider the impact of perturbing our initial parameters: $\alpha$, $\lambda$, $a$ and $b$. 
    %        \begin{figure}[ht]
    %        \begin{subfigure}{.49\textwidth}
    %            \centering
    %            \includegraphics[width=\linewidth]{Figures/Price_plot_0.8_0.7_0.18_0.92.pdf}
    %            \caption{$\lambda = 0.8$} 
    %            \label{fig:price_plot_1}
    %        \end{subfigure} 
    %        \hfill
    %        \begin{subfigure}{.49\textwidth}
    %            \centering
    %            \includegraphics[width=\linewidth]{Figures/Price_plot_0.9_0.7_0.12_0.92.pdf}
    %            \caption{$a = 0.12$} 
    %            \label{fig:price_plot_2}
    %        \end{subfigure}
    %        \begin{subfigure}{.49\textwidth}
    %            \centering
    %            \includegraphics[width=\linewidth]{Figures/Price_plot_0.9_0.7_0.18_0.2.pdf}
    %            \caption{$b = 0.2$} 
    %            \label{fig:price_plot_3}
    %        \end{subfigure}
    %        \hfill
    %        \begin{subfigure}{.49\textwidth}
    %            \centering
    %            \includegraphics[width=\linewidth]{Figures/Price_plot_0.9_0.01_0.22_0.92.pdf}
    %            \caption{$\alpha = 0.01, a = 0.22$} 
    %            \label{fig:price_plot_4}
    %        \end{subfigure}
    %        \caption{\textbf{Price Dynamics}; these four plots demonstrate the changes in the price dynamics after slight alternations of our initialization parameters. The baseline parameters are $\lambda = 0.9$, $\alpha = 0.7$, $a = 0.18$, $b = 0.92$. The alterations in each figure is noted in the caption.}
    %        \label{fig:price_dynamics}
    %    \end{figure} 

    %Figures in \ref{fig:price_dynamics} reproduce Figure \ref{fig:price_baseline} with slight changes to demand parameters. In all cases, some initial price increase remains. The qualitative results are broadly summarised as follows: i) a decrease in responsiveness through $\lambda$ lowers volatility, as expected from the derived dynamics, ii) lower momentum $a$ removes the oscillations, as investors are less likely to seize on the direction of price swings, iii) lower aversion to volatility through $b$ yields larger oscillations, and iv) even with minimal weight on average sentiment in $\alpha$, the historical experiences of each individual alone can produce rich dynamics, as we see by increasing $a$. However, the social component is important in driving an initial run up in price, which is intuitive; new hype investors do not have any experience to rely on when deciding whether to buy or sell. In the end, cross-sectional and temporal heterogeneity likely play a compounding role.
    
    % \clearpage

==> Appendices/Topic_model.tex <==
\subsection{Topic model}
\label{app:topic_model}

         \begin{figure}[ht]
             \begin{center} 
                 \includegraphics[width=\textwidth]{Figures/topic_model.pdf} 
                 \caption{\textbf{Temporal trends in topics}; the stacked count, normalized to 100\% at each time period, showing the prevalence of a select subset of topics discussed on WallStreetBets.}
                 \label{fig:topic_hist}
             \end{center}
         \end{figure} 

        Does WSB reflect new information for the larger market to trade on, or social activity that drives perceived changes in value, regardless of fundamentals? A topic model offers a simple method to evaluate the content of WSB discussions. Figure \ref{fig:topic_hist} presents our preferred topic model, namely the Biterm Topic Model (BTM), which is optimal for smaller bodies of text \citep{yan2013biterm}. Submissions from April 2012 to February 2021 give a time series of almost 100 months. A random sample of submissions is drawn for the months of January and February 2021 in order to prevent these two months, with a high number of submissions, from skewing the topic model results. 
        
        Figure \ref{fig:topic_hist} presents a stacked plot of the monthly submission count of a selected subset of discussions, normalised by the total across the selected topics. It begins in 2015 when the forum gained a consistent user base. On one hand, some topics persist in the overall discussion: people consistently ask for advice about trading accounts and anonymously share details of how their trading is affecting their personal lives. On the other hand, topics concerned with larger economic trends wax and wane over the observation period. Two examples of this are the uptick in submissions discussing GME and Roinhood account trading limits, coinciding with the GME short squeeze, and the COVID-19 topic, which is negligible until January 2020, but gains prominence in the subsequent months. Pharmaceutical company and natural resource discussions, on the other hand, seem to loose popularity. A full list of topics with their respective keywords is presented below.
        
\clearpage

\input{Tables/topic_model1}
\input{Tables/topic_model2}

==> Appendices/bifurcation_diagrams_alpha.tex <==
\subsection{Bifurcation diagram with respect to consensus}
\label{app:bifurcation_alpha}

    \begin{figure}[!htbp]
        \begin{subfigure}{\textwidth}
            \centering
            \includegraphics{Figures/Simulation/phi_bifurcation_high_beta.png}
            \caption{$C = 2.5$} 
            \label{fig:phi_bifurcation_diagram_high_beta}
        \end{subfigure}

        \begin{subfigure}{\textwidth}
            \centering
            \includegraphics{Figures/Simulation/return_bifurcation_high_beta.png}
            \caption{$C = 2.5$} 
            \label{fig:return_bifurcation_diagram_high_beta}
        \end{subfigure}
        
        \begin{subfigure}{\textwidth}
            \centering
            \includegraphics{Figures/Simulation/phi_bifurcation_low_beta.png}
            \caption{$C = 0.3$} 
            \label{fig:phi_bifurcation_diagram_low_beta}
        \end{subfigure}

        \begin{subfigure}{\textwidth}
            \centering
            \includegraphics{Figures/Simulation/return_bifurcation_low_beta.png}
            \caption{$C = 0.3$} 
            \label{fig:return_bifurcation_diagram_low_beta}
        \end{subfigure}
        
        \caption{\footnotesize{\textbf{Bifurcation diagrams with respect to consensus parameter $\alpha$}; the final values from one thousand iterations of the dynamic system in Eqs. \ref{eq:consensus_model_discrete_1}-\ref{eq:consensus_model_discrete_2}, are plotted, for two values of $C$ (2.5 and 0.3) and a range of values for $\alpha$ between zero and two. Remaining parameters are constant for $\beta = 1$ and $\lambda = 1$. One hundred initial values for $r$ are drawn from a normal distribution with mean zero and variance 0.25, with $\phi$ initiated at zero.}}
        \label{fig:bifurcation_diagram_alpha}
    \end{figure} 
    
    We produce two additional bifurcation diagrams for each state variable, varying $\alpha$. Figure \ref{fig:stability_regions} suggests two interesting values for $C$ -- one at 0.3, and a second at 2.5. We assign parameter $\beta$ a value of one. We then initialise sentiment $\phi_0$ to be zero, and randomly draw one hundred values for returns $r_0$ from a normal distribution with mean zero and variance 0.25. For a set of values of $\alpha$, ranging from zero to two, we iterate forward $\phi_t$ and $r_t$ one thousand times. The final values for $\phi_t$ and $r_t$ are then plotted as a function of $\alpha$.
    
    Those plots are presented in Figure \ref{fig:bifurcation_diagram_alpha}. Figure \ref{fig:phi_bifurcation_diagram_high_beta} illustrates the final values for $\phi_t$ when $C$ is set to 2.5, and Figure \ref{fig:return_bifurcation_diagram_high_beta} does the same for $r_t$. For low values of $\alpha$, sentiments, and concurrently returns, display quasi-periodic dynamics (in the clouded regions), interrupted by stable cycles (for example when $\alpha$ is around 0.8). Larger values of $\alpha$ eventually dominate the effect of hype investors' large capacity, and the system settles at it steady states, with either positive or negative sentiment. This in stark contrast to a scenario where capacity is too small, as in Figures \ref{fig:phi_bifurcation_diagram_low_beta} and \ref{fig:return_bifurcation_diagram_low_beta} where $C$ is set to 0.3. The meaningful change in the behaviour of the system is that sentiments settle at one value, either positive or negative, when $\alpha$ is greater than one -- already present in the one-dimensional hyperbolic tangent map from Figure \ref{fig:bifurcation_1_D}. It is interesting to note that there is slight residual dispersion in returns in Figure \ref{fig:return_bifurcation_diagram_low_beta} (note the scale of the axis) when $\alpha$ reaches that threshold, as one steady state loses its stability, and two new ones barely emerge.

==> Appendices/old/Consensus_network.tex <==

\subsection{Aggregate Opinion Formation}
\label{app:consensus_network}

        \input{Tables/leontieff_sentiment_spillovers}
        
        One pertinent question is on the persistence of aggregate opinions. This is of particular importance when considering market impact: do investors come to an agreement about whether an asset should be bought or sold? We estimate this phenomenon through a parameter $\alpha$, which denotes the aggregate buying/selling intensity resulting from individual opinion formation.
        
        One way gauge $\alpha$ is to replace matrix $\boldsymbol{W}$ in Eqs. \ref{eq:network_model1}-\ref{eq:network_model2} by its Leontief inverse, $(\boldsymbol{I}-\boldsymbol{W})^{-1}$. Instead of a weighted average of $i$'s direct neighbours, the Leontief inverse returns the overall position of user $i$ in the network. While immediate neighbours are still highly weighted, the sentiments of their neighbours, and those neighbours' neighbours, feature as well. The end result is that $(\boldsymbol{I}-\boldsymbol{W})^{-1}$ captures the sentiments related to an asset in the broader context of the whole forum, appropriately discounting those further removed from $i$.
        
        The first two columns in Table \ref{tab:leontieff_sentiment_spillovers} show the coefficients of Eq. \ref{eq:network_model2}, but with the adjacency matrix replaced by its Leontief inverse, and the diagonal elements set to zero. The baseline coefficients are suppressed, since they do not vary substantially from Table \ref{tab:adjacent_sentiment_spillovers}. The stark difference here is the much stronger effect of volatility, $(\boldsymbol{I}-\boldsymbol{W})^{-1} \sigma$. It reflects a strong persistence of bearish sentiments in discussions when the asset in question experiences volatility. In contrast to the statistically insignificant coefficient on overall returns, $(\boldsymbol{I}-\boldsymbol{W})^{-1} R^e$, volatility, and the panic it appears to induce, has a powerful, propagating effect in the formation of investor opinions in WSB.
        
        The final set of columns in Table \ref{tab:leontieff_sentiment_spillovers} investigate whether sentiments detected in users who post their first submission, versus those that have already expressed an opinion in the past, are noticeably different. The answer is affirmative; interacting the relevant dummy variable with the spillover term, $(\boldsymbol{I}-\boldsymbol{W})^{-1} \boldsymbol{\phi^s} \times \phi^{NA}_{-1}$, demonstrates that the large bearish spillovers take hold in users who post for the first time. The original coefficient, $(\boldsymbol{I}-\boldsymbol{W})^{-1} \boldsymbol{\phi^-}$, is statistically insignificant in predicting bearish over neutral sentiment, while those for bullish sentiment are largely in the same direction.

==> Appendices/old/Data.tex <==
\newpage

\subsection{Data Appendix}
\label{app:data_appendix}

    Besides the scraped text data from Reddit, we downloaded historical price series on extracted tickers from The Center for Research on Security Prices (CRSP). The time period, denoted by $t$, is defined as the 24 hours between closing times on the New York Stock Exchange, namely 4pm EST. For example, a submission made on Tuesday at 5pm EST is categorised in the same time frame as a submission made on the following Wednesday at 10am. This is done to mitigate any influence that news occurring outside market hours might have on WSB conversations. The choice of timing may not be consistent with non-US stock markets, but, given that almost all discussed assets are US stocks and indices, this does not impact our findings. The financial data used are: $P_{i,t}$, the dollar price of security $i$ at closing time of day $t$, $R^f_t$, the risk-free rate of return obtained from Kenneth R. French's data library, $(P^H_{i,t},P^L_{i,t})$, the intra-day high and low prices of security $i$ at closing time of day $t$, and $V_{i,t}$, the trading volume of security $i$ at closing time of day $t$.
    
    We computed the variables for Table \ref{tab:submission_time_series_regression} as follows:
    
    \begin{itemize}
        \item $R^e_{i,t} = \mathbb{E}_t\left[ \frac{P_{i,d \in t}}{P_{i,d-1}} - (1+R^f_{d \in t}) \right]$, where $d$ is a day in calendar week $t$, $P_{i,d}$ is the closing price of asset $i$ on day $d$, and $R^f_d$ is the daily risk free rate on day $d$,and $\mathbb{E}_t$ computes the arithmetic mean of price returns across days $d$ in week $t$,
        \item $\sigma^e_{i,t} = \sqrt{\mathbb{VAR}_t\left[ \frac{P_{i,d \in t}}{P_{i,d-1}} - (1+R^f_{d \in t}) \right]}$, where $d$ is a day in calendar week $t$, and $\mathbb{VAR}_t$ computes the variance of price returns across days $d$ in week $t$,
        \item $Q_{i,t} = \mathbb{E}_t\left[ P_{i,d \in t} V_{i, d \in t} \right]$, where $V_{i,d}$ is the trading volume, in billions, of asset $i$ on day $d$.
    \end{itemize}
    
    We calculated the variables used in Table \ref{tab:adjacent_sentiment_spillovers} as follows:
    
    \begin{itemize}
        \item $R^e_{i,t} = \frac{P_{i,t}}{P_{i,t-1}} - (1+R^f_t)$, where $P_{i,t}$ is the closing price of asset $i$ on day $t$, and $R^f_t$ is the daily risk free rate on day $t$,
        \item $\widetilde{R^e_{i,t}} = \frac{P_{i,t-1}}{P_{i,t-6}} - (1+R^f_{t-6})^5$, where the 5-period lag is based on a 5-day trading week,
        \item $\sigma_{i,t} = \sqrt{\frac{1}{10}\sum_{k=1}^{11} (R^e_{i,t-k} - \overline{R^e}_{i,t-1})^2}$, where $\overline{R^e}_{i,t}$ denotes the average excess return observed between days $t$ and $t-10$,
        \item $\boldsymbol{W}$ is the normalised submission adjacency matrix, where $w_{i,j}$ is equal to the number of comments made by $i$'s author on an older submission $j$ with the same extracted ticker, divided by the total number of comments made by $i$'s author on older submissions with the same extracted ticker,
        \item $\phi^s$ denotes a dummy variable for a submission with sentiment $s$, where $s$ can be bullish ($s = +1$), bearish ($s = -1$) or neutral ($s = 0$),
        \item $\phi^s_{-1}$ denotes a dummy, as above, for the sentiment of the last post made by the author on the same extracted ticker, where $\phi^{NA}_{-1}$ represents the lack of such a submission.
    \end{itemize}
    
    We took two extra cleaning steps. First, to account for stock splits and mergers, we use CRSP's cumulative factors to adjust prices and volumes for each security $i$. Second, we remove any instances where the price is negative, or the excess return is greater than 10.

==> Appendices/old/Model_30_Jan_2023.tex <==
\section{Social dynamics and asset prices}
\label{sec:model}

Sharing investment strategies appears self-defeating, so what motivates retail investors to do so online, in such an unabashed manner? We study their interactions through an asset demand model, by incorporating information complementarities in investment decisions. These give rise to \textit{social contagion} in asset demand; investors buy the asset because others do as well, irrespective of their personal beliefs. This behaviour, if significant, can create reversals in asset price returns. 

The mechanism is motivated by a recent literature that studies diagnostic expectations \citep{bordalo2021diagnostic}. In doing so, investors trade on the momentum of the stock price, against a supply of shares provided by noise traders.  Our inclusion of a social component subsequently induces persistence in asset demand over time, which leads to reversal in future returns after an increase in price.

\subsection{General setup}
\label{subsec:asset_demand}
We analyse prices in each period $t$ for one asset traded by $N$ investors, indexed by $i$. Each investor derives CARA utility from consuming $c$, $U_i(c_i) = \text{exp}(-\gamma c_i)$, where $\gamma$ is the constant absolute rate of risk aversion. We do not include any discounting in their decision-making, but assume they evaluate the asset according to a forward-looking value $V$ with expectation $\mathbb{E}_i(V)$.

For now, we drop the time subscript to study a static version of the model. Shares $\phi_i$ are purchased at current market price $p$ to optimise the mean-variance objective function \begin{align}
\label{eq:mean_variance_tradeoff}
    \mathcal{L}(\phi_i) &= [\mathbb{E}_i(V) - p]\phi_i - \frac{\gamma}{2}\mathbb{E}_i(V - p)^2\phi_i^2, \\
    \Rightarrow \phi_i^\ast &= \frac{\mathbb{E}_i(V) - p}{\gamma \mathbb{E}_i(V - p)^2},
\end{align}
where an asterisk denotes the value that maximises objective $\mathcal{L}$. In this way, we distinguish between beliefs about value $\mathbb{E}_i(V)$ from investor $i$'s decision to buy amount $\phi_i$. 

\paragraph{Simple price equilibrium} We assume that asset supply originates from noise traders, as in \citet{bordalo2021diagnostic}, to find a price equilibrium. In effect, equilibrium demands $\sum \phi_i^\ast$ sum to exogenous supply $S$. Assuming fixed uncertainty $\sigma^2 = \mathbb{E}_i(V - p)^2$ and averaging expected values $\mathbb{E}(V) = {1}/{N} \sum \mathbb{E}_i(V)$ yields the following expression for the equilibrium price:
\begin{align}
    p = \mathbb{E}(V) - \frac{S}{N} \gamma \sigma^2. \label{eq:simple_equilibrium}
\end{align}
Eq. \ref{eq:simple_equilibrium} accounts for the price level by investor's average expected value of the asset, in addition to their ability to absorb the exogenous level of assets supplied. This ability depends on the depth of the investor pool -- reflected by the number of investors $N$ -- as well as their risk appetite $\gamma \sigma^2$. In this simple market, the price increases with expected value, and decreases with supply.

This expression for prices also ignores heterogeneity and aggregation. Eq. \ref{eq:simple_equilibrium} mimics a single representative investor with some demand size $N$. However, strategic interactions may give rise to feedback loops in investor demands that do not average out. We also do not consider the effect of heterogeneity in investor wealth, or other size metrics, although the model can be extended for that purpose. Investors central in a social network are `indirectly' large by their ability to sway others. [GABAIX]

The first goal of this section is to endogenise investors' expectation formation for value $\mathbb{E}_i(V)$, and determine a trajectory for prices when aggregating these components. A long literature investigates the link between subjective asset price beliefs and prices, and our contribution is to include a term for social learning. The second goal is to investigate this equilibrium price in a dynamic setting where values are updated under some extrapolation.

\subsection{Static model with information complementarities} 
We study the role of information complementarities in investors' beliefs about the value of an asset. Investor $i$'s maximised payoff from Eq. \ref{eq:mean_variance_tradeoff} is
\begin{align}
    \mathcal{L}(\phi_i^\ast) &= \frac{1}{2\gamma} \frac{\mathbb{E}_i^2(V-p)}{\mathbb{E}_i(V-p)^2} \\
    % &= \frac{1}{2\gamma} \left(1 - \frac{\mathbb{E}_i[\mathbb{E}_i(V) - V]^2}{\mathbb{E}_i(V-p)^2}\right),
    &= \frac{1}{2\gamma} \left(1 - \frac{\sigma_i^2(V)}{\mathbb{E}_i(V-p)^2}\right),    
\end{align}
where $\sigma_i^2$ denotes investors' variance for value $\sigma_i^2(V) = \mathbb{E}_i(V^2) - \mathbb{E}_i^2(V)$. At this optimised level, payoffs decrease as uncertainty about value $V$ increases, to the extent that squared returns themselves are low. This expression demonstrates the value of social networking. If investors start with different signals about the asset's value, the ability to aggregate them by listening to others improves the precision of their expectation, and their final expected payoff. In this stage, prices themselves do not feature. Investors benefit from a better estimate of value $V$ at any price $p$.

The extent to which uncertainty on the difference between realised price from the expected value $\mathbb{E}_i(V-p)^2$ is significant remains unclear. Investors expect the price to be a realisation of aggregated expected value and a mean zero, unobserved supply shock $S$. The difficulty in finding a market-clearing price lies in the non-linear aggregation of demand. Price is not linear in the expectations of value, nor in the uncertainty faced by individuals.

To circumvent this problem, we assume a specific form for investors' price uncertainty:
\begin{align}
    E_i(V - p)^2 = \sigma_i^2(V) + \sigma_i^2(s),
\end{align}
where $\sigma_i^2(s)$ corresponds to the variance of supply shock $S \gamma \sigma^2 /N$ in Eq. \ref{eq:simple_equilibrium}. This form for uncertainty corresponds to an investor who based their price expectations on a form of the simple equilibrium in Eq. \ref{eq:simple_equilibrium}, but uses their expected value as the aggregate, and does not adjust their 


An investor's expectation includes some signal $b_i$, with information both public and private to $i$, and asset demand by other investors $\phi_{-i}$:
\begin{align}
    \mathbb{E}_i(V) = g(b_i) + f(\phi_{-i}).
    \label{eq:quadratic_loss}
\end{align}
We assume that functions $g(\cdot),f(\cdot)$ are monotonic and continuous, but are specifically interested in the form of $f(\cdot)$. Eq. \ref{eq:quadratic_loss} is a well-known formulation for strategic interactions between agents acting under quadratic loss \citep{zenou2016key}. Definition \ref{definition:complementariy} establishes the notion of complementary investment in this context.

\input{Cells/1_Definition}

The complementarity in asset demand between investors comes from the aggregation of idiosyncratic information on the value of the asset. Investor $i$ is motivated to better inform their decision by gleaning information from their peers' actions. Thus, if they believe the value is low due to their personal signal $b_i$, higher purchases by their friends would lead them to revise their decision to buy a low amount of the asset. The investor in question may have simply drawn a bad signal. Here, we simplify the analysis by assuming that each investor's information aggregation method is an arithmetic mean of others' investment demand. The asset's expected value increase linearly in this `social' component. Information acquisition under complementary decisions is studied in detail by \citet{hellwig2009knowing}.

\paragraph{Strategic complementarities and peer effects.}
What compels retail investors to share strategies via WSB? We suggest one answer by appealing to \cites{hellwig2009knowing} main result, which we rewrite in Proposition \ref{proposition:strategic_interactions}. In addition to the quadratic loss assumed in Eq. \ref{eq:mean_variance_tradeoff}, we remind the reader of the additional assumptions in their framework, adapted to the present context.
\input{Cells/1_Assumption}
\input{Cells/2_Assumption}
\input{Cells/1_Proposition}

Proposition \ref{proposition:strategic_interactions} predicts that interactions between investors whose decisions include a social component (a group we call `hype investors') provide them with additional expected utility. This, in turn, increases their propensity to invest according to their updated sentiment, under costly information acquisition. We empirically validate whether Proposition \ref{proposition:strategic_interactions} holds in the context of WSB and, thereby, study the social aspects of investing. 

\subsection{Price dynamics with peer effects} 

To study the joint dynamics of an asset's price and demand by social investors, we treat demand $\phi$ and price $p$ as state variables for a dynamic system, indexed by time $t$. In doing so, we assume that demands $\phi_{i,t}$ are updated using signals $b_{i,t}$ and past demand $\phi_{t-1}$. Aggregate asset demand and price are
\begin{align}
    \phi_t &= \frac{\mathbb{E}_t[g(b_{i,t})] + \alpha \phi_{t-1} - p_t}{\gamma \sigma^2}, \label{eq:demand_system} \\
    p_t &= \mathbb{E}_t[g(b_{i,t})] + \alpha \phi_{t-1} - \frac{S_t}{N}\gamma \sigma^2, \label{eq:price_system}
\end{align}
which demonstrate the importance of signals $b_{i,t}$ in determining the trajectory of demand. Studies in behavioural finance suggest several components that ultimately deviate from rational expectations. In this instance, demand depends on it's lag. We believe this accurately reflects the nature of discussions on WSB specifically, which is characterised by `leaders' who garner followers to adopt their positions. 

% \paragraph{Rational Expectations.} For the simplest scenario, we make the first assumption that investors value the asset according to its expected future price, so that $\mathbb{E}[g(b_{i,t})] = \mathbb{E}_t(p_{t+1})$. This leaves us with an easy system to analyse:
% \begin{align}
%     \phi_t &= \frac{\mathbb{E}_t(r_{t+1}) + \alpha \phi_{t-1}}{\gamma \sigma^2}, \\
%     \mathbb{E}_t(r_{t+1}) &= - \alpha \phi_{t-1} + \gamma \sigma^2 \phi_t ,
% \end{align}
% where return $r_t \equiv p_t-p_{t-1}$. The expression for returns in terms of asset demand can be simplified to 
% \begin{align}
%     \mathbb{E}_t(r_{t+1}) = \gamma\sigma^2 \Delta \phi_t + (\gamma\sigma^2 - \alpha) \phi_{t-1},
% \end{align}
% where $\Delta x_t \equiv x_t - x_{t-1}$. 

\paragraph{Mechanical Extrapolation.} We assume that investors partially trade on the momentum of the asset's price, which \citet{bordalo2021diagnostic} term `mechanical extrapolation'. The functional form of $\mathbb{E}[g(b_i)]$ is specified in Assumption \ref{assumption:mech_extrapolation}.

\input{Cells/1.1_Assumption}

Mechanical extrapolation is our preferred way to introduce a relationship between prices and demand \citep{barberis2018extrapolation}. A model with mechanical extrapolation has several shortcomings, one of which is the inability to relate expectation updates to psychological underpinnings. However, our assumption is justified by our empirical work in Section \ref{sec:consensus_results} which demonstrates that individuals update their outlook based on recent asset returns. 

\paragraph{System for price and demand.} Substituting Eq. \ref{eq:mech_extrapolation} into Eqs. \ref{eq:demand_system}-\ref{eq:price_system} yields demands and prices
\begin{align}
    \phi_t &= \frac{\alpha \phi_{t-1} + \beta r_t}{\gamma \sigma^2}, \\
    r_t &= -\frac{\alpha}{\beta} \phi_{t-1} + \frac{S_t\gamma \sigma^2}{\beta N}.
\end{align}
In this scenario, asset demand and returns are determined simultaneously. The first mechanism is through market clearing, where demand has to adjust to supply. The second is the adjustment of the expected value for the asset to the realised return through $\beta$ and the social signal through $\alpha$. As a result, returns are accounted for by current and past asset demand:
\begin{align}
\label{eq:return_against_demand}
    r_t = \frac{\gamma\sigma^2 }{\beta} \phi_t - \frac{\alpha}{\beta} \phi_{t-1}.
\end{align}
% \begin{align}
%     r_t = \frac{\gamma\sigma^2 }{\beta}\Delta \phi_t + \frac{\gamma\sigma^2 -\alpha}{\beta} \phi_{t-1}.
% \end{align}
This equation for asset demand in equilibrium offers three valuable insights. First, it requires a non-zero degree of extrapolation $\beta > 0$, otherwise demand does not adjust to price. Investors are never compelled to change their purchases since they believe the current price precisely reflects value. Second, higher demand increases current returns, but leads to a subsequent reversal in the following period. This is because the equilibrium price needs to satisfy the value expected both from extrapolation, in addition to the value estimated from the social components. Under exogenous supply, a strong positive signal from peers means that the extrapolated return is \textit{less} important in justifying a higher price. In equilibrium, this results in a negative relationship between returns and the lag in asset demand.

The reversal in returns is an important feature that emerges from social contagion in investors' price expectations. If large enough, these can produce bubbles in asset prices: initial momentum from positive news creates a price run-up, before an absence of news creates a drought of new asset demand. The subsequent price crash carries on its own momentum. We can treat demand as a latent variable to see these oscillations manifest in return data. Substituting lagged demand into the equation for returns, and iterating infinitely yields
\begin{align}
\label{eq:return_time_series}
    r_t = -\sum_{T = 1}^\infty \left(\frac{\alpha}{\gamma \sigma^2}\right)^T r_{t-T} + \frac{S_t\gamma \sigma^2}{\beta N}
\end{align}
as long as $\alpha / \gamma \sigma^2 < 1$, so that the contribution of demand fluctuations to returns converges to zero over time. This is an autoregressive model with infinite lags, where the coefficients decrease exponentially with lag size $T$. Without any knowledge of asset demand, the second term encapsulates an unobservable error term which the model links to exogenous changes in the asset's supply. Eq. \ref{eq:return_time_series} demonstrates that an exogenous increase in returns at time $t$ is followed by an smaller decrease in $t+1$. This oscillation persists indefinitely, and would converge to zero rapidly if the social signal $\alpha / \gamma \sigma^2$ is sufficiently small.

\subsection{Full model with fundamental traders.} 
\label{sec:model_bubbles}

The previous section proposes a simple model for how an economy with a single investor type, who extrapolate past price movements and leverage the sentiment of peers to determine asset demand. This model informs the potential relationship we can expect between returns and observed investor sentiment online. However, how would asset prices dynamically evolve in an economy with both `fundamental' traders and those who trade based on sentiment (formed from peers and extrapolation)? We further develop a model from \cite{barberis2018extrapolation} to understand how market dynamics might develop.

\paragraph{Investor price expectations} We begin with the same investment setting as \cite{barberis2018extrapolation}. We consider an economy with T + 1 dates. There are two assets: one risk-free and one
risky. The risk-free asset earns a constant return which we normalize to zero. The risky asset has a fixed supply of Q shares, and each share is a claim to a dividend $D_T$ paid at
the final date, T. The value of D is determined by $D_0$, a final dividend paid at time T whose value is known, and $N(0, \sigma^2_{D})$, which is i.i.d. noise realize at each time period. The price of the risky asset, $P_t$, is determined endogenously. There are two types of traders in the economy: fundamental traders and `hype' investors whose investment decisions are marked by $F$ and $H$. The time $t$ per capita demand of fundamental traders for shares of the risky asset is:
\begin{align}
    \frac{D_t - \gamma\sigma^2_{D} (T-t-1)Q - P_t}{\gamma\sigma^2_{D}},
\end{align}
where $D_t$ is the sum of $D_0$ and realized shocks to the dividend up to time $t$ and $\gamma$ is the trader's risk aversion. This expression is consistent with an investor who maximises a CARA utility defined ove r the next period's wealth.  

Hype investor demand, on the other hand, place some weight on the fundamental signal, but also place some weight on past price changes and the sentiments of others (in an effort to reach strategic information complementarities, as described in \cite{hellwig2009knowing}:

\begin{align}
    w_H \frac{D_t - \gamma\sigma^2_{D} (T-t-1)Q - P_t}{\gamma\sigma^2_{D}} + (1 - w_H)\frac{X_t}{\gamma\sigma^2_{D}},
\end{align}
where $X_t$ is the `hype' signal at time $t$. We propose two versions of the hype signal: i) where the hype investor updates his demand based on past stock returns and the observed sentiments of other investors, $X_t^d$, and ii) where the the hype investor updates his belief about the future price change of the stock, rather than demand, $X_t^b$. Both models are of interest since the former is more directly comparable to the literature, while the latter is closer to the parameters we can estimate from the data. 

$X_t^d$ is updated as follows:
\begin{align}
    \label{eq:X_update_demand}
    X_{t}^d = \theta_d X_{t-1}^d + (1-\theta_d)S_t,
\end{align}
where $S_t$ is the investor sentiment composed of the observed sentiment of peers in the previous time step, $S_{t-1}$, and the observed price change, $P_{t-1} - P_{t-2}$,
\begin{align*}
    S_t = w_E(P_{t-1} - P_{t-2}) + w_S(S_{t-1}).
\end{align*}
This modeling choice implies that individual demand is driven not only by changes in price, but also in how fellow hype investors react. The model also gives additional flexibility to explore how assets might react to a purely socially-driven shock, rather than only a new-driven one.

 $X_t^b$ is updated as follows:
\begin{align}
    \label{eq:X_update_belief}
    X_{t-1}^b = \theta_b B_{t-1} + (1-\theta_b)S_t,
\end{align}
where $S_t$ is defined as before, but the investor updates their entire belief about the change in asset price, rather than only the `hype' part of his belief,
\begin{align*}
    B_t = w_H \frac{D_t - \gamma\sigma^2_{D} (T-t-1)Q - P_t}{\gamma\sigma^2_{D}} + (1 - w_H)\frac{X_t^b}{\gamma\sigma^2_{D}}.
\end{align*}
In the formulation with beliefs, we are able to measure the expressed sentiments of investors online over time and estimate $\theta_b$ based on the information they are exposed to and how their sentiment is updated. This is not possible when we do not explicitly estimate the investor belief, as in the formulation in \ref{eq:X_update_demand}.

\paragraph{Determining a market-clearing price.} As in \cite{barberis2018extrapolation}, we propose a short sale constraint to establish the market-clearing price, where the quantity demanded by both types of traders is bounded at zero:
\begin{align}
    \label{eq:short_sale}
    N_t^F &= max \left[   \frac{D_t - \gamma\sigma^2_{D} (T-t-1)Q - P_t}{\gamma\sigma^2_{D}}, 0 \right], \\
    N_t^H &= max \left[  w_H \frac{D_t - \gamma\sigma^2_{D} (T-t-1)Q - P_t}{\gamma\sigma^2_{D}} + (1 - w_H) \left(\frac{X_t}{\gamma\sigma^2_{D}} \right) , 0 \right].    
\end{align}
We use this formulation to calculate the price at which the short-sale constraint begins to bind for each type of trader -- at this price the trader would be indifferent between staying in or leaving the market:
\begin{align}
    \label{eq:market_clearing}
    P_t^F &= D_t - \gamma\sigma^2_{D} (T-t-1)Q - P_t, \\
    P_t^H &= D_t - \gamma\sigma^2_{D} (T-t-1)Q - P_t + \frac{(1 - w_H)}{w_H} \left(\frac{X_t}{\gamma\sigma^2_{D}} \right). 
\end{align}
Finally, we calculate the total demand at both price points, $P_t^F$ and $P_t^H$. If the quantity demanded at both price points is below Q, the total number of shares available, we determine the price as if both types of traders were in the market -- as shown in Eq. \ref{eq:bubble_price1}. Otherwise, we determine the price as if only hype traders were in the market, as in Eq. \ref{eq:bubble_price2}:
\begin{align}
    \label{eq:bubble_price1}
    P_t &=  D_t + \frac{\mu_H(1-w_H)}{\mu_F+\mu_H w_H} X_t - \gamma \sigma_D^2 Q \frac{(T-t-1) (\mu_H w_H + \mu_F) + 1}{\mu_H w_H + \mu_F},\\ 
    \label{eq:bubble_price2}
    P_t &=  D_t + \frac{\mu_H(1-w_H)}{\mu_H w_H} X_t - \gamma \sigma_D^2 Q \frac{(T-t-1) (\mu_H w_H) + 1}{\mu_H w_H}.
\end{align}

\paragraph{Bubbles and peers}

We compare the price dynamics across different models for bubbles. As a first baseline model, we consider the market price if all traders were fundamental traders. The market clearing price would be: 
\begin{align*}
    D_t - \gamma \sigma_D^2(T-t-1)Q.
\end{align*}
As a second baseline, we consider the model from \cite{barberis2018extrapolation}, which is similar to our model in for $X_t^d$ in Eq. \ref{eq:X_update_demand}. We look to compare our two baseline models to our model for hype investor demand, where $X_t^d$ is updated as in Eq. \ref{eq:X_update_demand}, and our model for hype investor beliefs, where $X_t^b$ is updated as in Eq. \ref{eq:X_update_belief}.


    \begin{figure}[!ht]
        \centering
        \includegraphics[width = 0.95\textwidth]{Figures/3_Model/bubbles1.pdf}
        \caption{\footnotesize{\textbf{Bubbles with Hype Investors:} We present the price evolution for an asset in several settings: i) with only 
 fundamental traders are present, ii) with fundamental traders and extrapolators \citep{barberis2018extrapolation}, iii) with fundamental traders and hype traders who update their demand, and iv) with fundamental traders and hype investors who update their beliefs. We observe the asset over 50 time periods (T=50), which has $D_0 = 100$ and experiences 10 shocks of zero, followed
by shocks of 2, 4, 6, followed by 37 shocks of zero to its dividend. We assume 30\% of traders are fundamental traders, $\mu_F$, and 70\% are non fundamental, $\mu_H$ (except for the \textit{Fundamental Traders} model, where all traders are assumed to be fundamental). Other parameters in the model are: $\sigma_D = 3$, $\gamma = 1$. For the models of \textit{Extrapolators} and \textit{Hype Investor - Demand Update}, we set $\theta$ and $\theta_d$ to 0.9, and $w_i$ and $w_H$ to 0.1. For both hype investor models, we set $w_E$ and $w_S$ to 0.9 and 0.2, respectively, as shown by the data. For our model of \textit{Hype Investor - Belief Update} we set $\theta_b$ to 0.15, and $w_E$ to 0.6 as motivated by our data. }}
        \label{fig:bubbles1}
    \end{figure}

For our first experiments, presented in Figure \ref{fig:bubbles1}, we consider a setting similar to \cite{barberis2018extrapolation}. We observe 50-period
sequence of cash-flow shocks impacting the dividend at each time $t$ (T=50), where $D_0$ is known to be 100. The first ten shocks are all equal to zero, followed by three positive shocks (2, 4, 6), followed by 37 more shocks of zero. We motivate our choice of parameters for the models of hype investors by our observations from our empirical work in the following section. Specifically, we observe that investors place significant weight on the extrapolation and therefore set $w_E = 0.9$; they also update their perspectives based on peers and set $w_S = 0.2$. We are not able to observe how hype investors update their demand -- we therefore set $\theta_d = 0.9$ consistently with \cite{barberis2018extrapolation}, however, we are able to observe changes to their belief. We, therefore, estimate $\theta_b = 0.15$ -- showing that investors place a much greater weight on recent information than on their past beliefs. Finally, we observe that peer sentiments and recent extrapolation explain a fraction of how investors update their beliefs -- we, therefore, conclude that hype investors likely place a greater weight on fundamental signals than assumed in \cite{barberis2018extrapolation} and set $w_H = 0.6$ for our model with belief updates. 

There are several noteworthy observations from Figure \ref{fig:bubbles1}. A model with peers creates larger and more prolonged bubbles than that without - observable by comparing the model with \textit{Extrapolators} and \textit{Hype Investors - Demand Update}. This is unsurprising as price increases are driven not only by extrapolation, but also by peer reinforcement who reinforce the validity of the price increase. We also observe that our model with belief updates produces a much shorter price deviation. This is largely caused by the greater emphasis that traders in this model place on the fundamental value of the asset. We believe that this, however, seems like a plausible model -- the change in the dividend corresponds to a single shock over two standard deviations. Even though it is likely that the market might over-react in such a scenario, we would not necessarily expect a prolonged bubble from a single shock of this size. 

    \begin{figure}[!ht]
        \centering
        \includegraphics[width = 0.95\textwidth]{Figures/3_Model/bubbles_sentiment.pdf}
        \caption{\footnotesize{\textbf{Bubbles with Hype Investors:} We present the price evolution for an asset in several settings: i) with only 
 fundamental traders are present, ii) with fundamental traders and extrapolators \citep{barberis2018extrapolation}, iii) with fundamental traders and hype traders who update their demand, and iv) with fundamental traders and hype investors who update their beliefs. We observe the asset over 30 time periods (T=50), which has $D_0 = 100$ and experiences no dividend shocks, however, experiences positive peer sentiment shocks of 20 in periods 5,6,7. We assume 30\% of traders are fundamental traders, $\mu_F$, and 70\% are non fundamental, $\mu_H$ (except for the \textit{Fundamental Traders} model, where all traders are assumed to be fundamental). Other parameters in the model are: $\sigma_D = 3$, $\gamma = 1$. For the models of \textit{Extrapolators} and \textit{Hype Investor - Demand Update}, we set $\theta$ and $\theta_d$ to 0.9, and $w_i$ and $w_H$ to 0.1. For both hype investor models, we set $w_E$ and $w_S$ to 0.9 and 0.2, respectively, as shown by the data. For our model of \textit{Hype Investor - Belief Update} we set $\theta_b$ to 0.15, and $w_E$ to 0.6 as motivated by our data. }}
        \label{fig:bubbles2}
    \end{figure}

    For our second set of experiments, we would like to show how `animal spirits' or a random positive shock to peer sentiments can also drive bubbles. In Figure \ref{fig:bubbles2}, we show that several positive shocks to peer sentiment can, indeed, drive prices to deviate from fundamentals in our model. The individuals react more quickly, in our model with belief updates and the price returns to its fundamental value more rapidly, as hype traders place a greater emphasis on fundamental value. 

\subsection{Initial evidence}




==> Appendices/old/VAB_model.tex <==
\newpage

\subsection{Contagion Model}
\label{app:vab_model}

\paragraph{Contagion}
    We turn to an adapted Kermack-McKendrick SIR epidemic model to quantify the evolution of asset demand via social contagion, advocated in \citet{shiller2017narrative}. This choice is justified through our results in Section \ref{subsec:contagion} and empirically validated in Appendix \ref{app:vab_model}. We propose the following relationships between susceptible, $V$, active/infected, $A$, and recovered, $B$, investors in a specific asset:
    \begin{align}
    \label{eq:sir}
        \frac{dV}{dt} &= -cAV, \\
        \frac{dA}{dt} &= cAV -rA, \nonumber \\
        \frac{dB}{dt} &= rA, \nonumber
    \end{align}
    where $c$ is the contagion rate, and $r$ is the recovery rate. The total population of potential hype investors, $N=V+A+B$, is assumed constant. We take this model literally to understand contagion in asset interest on WSB. `Active' users forgo passive investment, adopt a specific position in an asset, and convince others to do the same. `Recovered' users lose interest and cease to believe in the hype, and thus close their asset-specific position. `Susceptible' users have not yet taken any investment action but could potentially become interested in the asset, as they seek investment advice from their peers. We use $A$ as an estimate for the number of hype investors in an asset at a certain point in time. 

\paragraph{Empirical evidence for the contagion model}
    
 %       \begin{figure}[ht]
 %                   \centering
 %                   \includegraphics[width=\textwidth]{Figures/VAB/all_ticker_activity.pdf}
 %                   \caption{\textbf{Ticker Activity versus Overall WSB Activity}; the number of unique monthly active users (users who comment or post) on the left y-axis plotted plotted against the unique number of posters about a specific ticker (on the right y-axis). Both are plotted as 3-month rolling means.}
 %                   \label{fig:contagion_activity2}
 %       \end{figure}

        \begin{figure}[ht]
            \begin{subfigure}[t]{.5\textwidth}
                \centering
                \includegraphics[width=\textwidth]{Figures/VAB/JNUG.pdf}
                \subcaption{JNUG}
                \label{fig:vab_jnug}
            \end{subfigure}
            \begin{subfigure}[t]{.5\textwidth}
                \centering
                \includegraphics[width=\textwidth]{Figures/VAB/MU.pdf}
                \subcaption{MU}
                \label{fig:vab_mu}
            \end{subfigure}  
            \bigskip
            \begin{subfigure}[t]{.495\textwidth}
                \centering
                \includegraphics[width=\textwidth]{Figures/VAB/SNAP.pdf}
                \subcaption{SNAP}
                \label{fig:vab_snap}
            \end{subfigure}  
            \hfill \hfill 
            \begin{subfigure}[t]{.495\textwidth}
                \centering
                \includegraphics[width=\textwidth]{Figures/VAB/TSLA.pdf}
                \subcaption{TSLA}
                \label{fig:vab_tsla}
            \end{subfigure}
            \caption{\textbf{Contagion Model Forecasts for Active Investors in Assets on the WSB Forum}; the contagion model is initialized with the parameters at the start of an `outbreak' of activity on WSB in a specific ticker and used to approximate the growing interest and, subsequent, loss of interest.}
            \label{fig:VAB_model_applied}
        \end{figure}
        We provide evidence that discussions about assets are self-perpetuating on WSB: social contagion appears to play a role in the assets that investors discuss and consider for their portfolios. Here, we attempt to reconcile the size of discussions on WSB over time with our contagion model of choice: the epidemiological SIR model.
        
    Figure \ref{fig:contagion_activity} shows that some of the most commonly mentioned tickers appear to exhibit a hump-shaped pattern of number of interested users over time. We use data from WSB to estimate our contagion parameters, $c$ and $r$, at different points in time and show that our simple contagion model captures the hump-shaped ticker interest. One challenge is that our epidemic model is well-suited to model a single `outbreak' in ticker interest, as it assumes a static population. We, therefore, look at how well our model fits data with non-overlapping periods of discussion intensity.
        
    Figure \ref{fig:VAB_model_applied} shows the \textit{predicted} discussion sizes of specific tickers from the contagion model (as a percent of active users on the forum at the time) versus the \textit{actual} sizes of ticker discussions on the WSB forum. Despite its clear shortcomings, this simple model that is tuned on noisy global parameters still captures the overall shape of social contagion in ticker interest. It exhibits some desirable properties, such as the fact that contagion spreads more slowly in communities that are sparse and faster as the community grows: consider Figure \ref{fig:vab_jnug} where JNUG interest gradually permeated the forum over the course of a year, whereas TSLA interest in 2020, displayed in Figure \ref{fig:vab_tsla}, spread to a much greater population over the course of three months.

\paragraph{Estimating $c$ and $r$ Parameters Globally}
        Certain contagion variables are more straightforward to estimate from WSB data than others. For the moment, we assume the total population at a given time, $N_t$, to be the number of active users on the forum: those who comment or post at time $t$. The number of users initially interested in asset $i$, $A_{i,0}$, is estimated as the number of people who post about $i$ in some starting period 0. The average dollar amount each user has at their disposal, $M$, can approximated from available surveys\footnote{\url{https://andriymulyar.com/blog/how-a-subreddit-made-millions-from-covid19}}. Model sensitivity is tested against all of these parameters. 
        
        Contagion parameters, $c$ and $r$, require more care in isolating the effect of social interaction from other variables that may impact asset interest. 
        
        The contagion rate is comprised of two parameters: 
        \begin{align}
            c = \tau \gamma,
        \end{align}
        where $\tau$ is transmissibility, the probability of transmission of asset interest given contact between a susceptible and active investor), and $\gamma$ the average rate of contact between susceptible and active investors on the forum. The first, $\tau$ is easily estimated from the results in Section \ref{subsec:contagion} (further detailed in \ref{app:matching}) showing a spread of ticker-specific interest at a rate of 1.1\% among tail tickers. In order to estimate $\gamma$, we counted the total number of unique users who commented on a submission, on average (this is an approximation for the number of `susceptible' individuals that an infected person comes in contact with), multiplied by the number of posts that a user makes, on average, about a given ticker, and divided by the number of users active on the forum, measured as unique users who post a submission or comment, while the submissions about the ticker are discussed on the forum. We consider interactions to be uniform over the duration of the `infectious period' so divide this number by the duration. The average contact rate is estimated at $\gamma = 1.2\times 10^{-4}\%$. This may seem particularly small, however, intuitively this is not surprising as $\gamma$ captures how many people will pay attention to a single submission versus all the other content in a thriving online community. The contact rate also differs greatly from one month to the next as people join and leave the forum, so this rate is more precisely tracked for each ticker that we estimate contagion for. This returns a combined contagion rate of $c = 9.8 \times 10^{-7}$.
        
        Estimating $r$ presents a challenge: users do not advertise a loss of interest in an asset on WSB. In order to estimate the recovery rate, we turn to its classic definition as `the inverse of the infectious period,' as described in \cite{ridenhour2018unraveling}. We consider the `infectious period' the time difference between when an author make his first post about a ticker and the time when his last post ceases to receive comments (ceases to be actively discussed on the forum). During this period, an individual spreads their perspective about an asset on the forum. We estimate the recovery rate at approximately $r = 1/19.6 = 5.1 \times 10^{-2}$. 
        
\paragraph{Initializing $c$, $r$, $N_0$ and $A_0$ for Social Contagion in a Specific Ticker}
        In order to estimate the contagion patterns presented in Figure \ref{fig:VAB_model_applied}, we tune the contagion parameters to be more precise for the ticker and time period in question. We initialize $N_0$ as the total number of unique authors who are active on the forum from the start to five months after the beginning of the contagion: we select this period in order to estimate the size of the population who would be affected by the excitement about a ticker, but we make the period sufficiently short so as to avoid capturing inflated population numbers driven by user churn (when a group of users becomes uninterested in a given subreddit and is replaced by a new group of users). One important shortcoming which results from this modeling choice is the fact that the model consistently over-estimates the number of infected individuals: our initial $N_0$ contains all posters and commenters on the forum; however, Section \ref{sec:data_method} establishes that there is an order of magnitude more comments than posts on the forum. Ultimately, we are interested in tracking posters in a given asset; this difference in populations results in consistent over-estimation. We initiate $A_0$, the initial population that begins to discuss a ticker on the forum driving further interest, as the average number of of unique authors posting about the ticker in the three months preceding the uptick. We also adjust $\gamma$ to be calculated at the time the uptick begins.

%\paragraph{Units and Further Discussion on Initialization of Parameters}

%We check our contagion units with the standard epidemeology literature and intuition. The change equations in Eq. \ref{eq:sir} should result in a unit of: $\frac{persons}{day}$. We consider our input into the $c$ constant; we know that $A,V$ have a units of $persons \times persons$, therefore our $c$ constant must have units of $\frac{1}{person-day}$. Our $c$ constant is composed of $\tau$ and $\gamma$. $\gamma$ helps us quantify how many contacts occur between $passive$ and $active$ individuals each day; $\tau$ tells us what proportion of the $passive$ investors become $active$ as a result. $\tau$ is a unitless constant as it is in persons who become $active$ divided by persons contacted in total, or $\frac{persons}{persons}$. The $\gamma \times AV$ should give us the total contacts between $passive$ and $active$ per day in units $\frac{person}{day}$. $\gamma$ should give us, for every $active$ individual, on a given day they are active, what is the probability that a $passive$ person comes in contact with them (in units of 1 divided by person $\times$ day)? Subsequently, $\gamma \times A$ would give us the number of $active$ investors that a single $passive$ investor comes into contact with each day. Finally, $\gamma \times AV$ would give us the total contacts between the two. We, therefore approximate $\gamma$ with this in mind. The $\gamma$ parameter is sometimes referred to as the fraction of $active$ individuals that a passive individual comes in contact with. However, on the WSB forum, the fraction of $active$ individuals is relatively small compared to the overall population. We therefore estimate the fraction of active individuals as the probability to come in contact with a single active individual (essentially discounting the probability that a $passive$ individual will encounter multiple $active$ individuals in a given day). This decision is justified both given how few $active$ individuals there are as compared to the overall size of the forum and given that in Figure \ref{fig:contagion_plot} we show that 71\% of people interact with one post before posting themselves. (or becoming $active$). We consider, over the duration of an $active$ individual posting on the forum, what fraction of the $passive$ population come in contact with this individual. We divide this by the total number of days that the activity lasts (to add a time dimension).

%\paragraph{Sensitivity of the Maximum of Active Investors to $c$, $r$}

%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=\textwidth]{Figures/VAB/beta_gamma_sensitivity.pdf}
%    \caption{\textbf{Sensitivity of $\text{max}(A)$ to $c$ and $r$ Parameters}; this plot shows the dependence of our $\text{max}(A)$ on various initialization parameters. This plot highlights that the current estimate lies at a point with a large gradient where $\text{max}(A)$ is not 0 but also not the entire population. This is consistent with empirical observations where not all investors become interested in a given asset - even for assets which are most popular on the forum. }
%    \label{fig:beta_gamma_sens}
%\end{figure}

%In our model, we are most interest in the number of \textit{active} investors, $A$, at a given point in time. This quantity approximates how many retail investors that are susceptible to social contagion are actively interested and investing in a given asset at a point in time. Specifically, we are interested in the $\text{max}(A)$ over the course of an entire ``social epidemic" as this would be tied to the maximum market impact that the social contagion would have. We, therefore consider how $\text{max}(A)$ varies with our initial $c$ and $r$ parameters. We initialize our model with the parameters in our second Tesla discussion, plotted in Figure \ref{fig:vab_tsla} and observe how $\text{max}(A)$ changes in the surrounding regions for $c$ and $r$, plotted in Figure \ref{fig:beta_gamma_sens}. We observe that as $r$ increases (which is the inverse of the duration for which an investor remains interested in a given asset) the $\text{max}(A)$ decreases: as people loose interest quickly, they have less time to spread their interest to others and, therefore, the excitement in the given asset dies out with very few active investors at a given point in time. We also observe that as $c$ increases, which is our contagion rate, the number of active investors at a point in time increases. A final important point is that a fairly rough approximation for the $c$ and $r$ parameters from our data place the estimate in a ``critical region" of the graph: a region with a high gradient - a region where not all investors on the forum become active in the specified asset. This is intuitive as we do not observe that all investors discuss a single asset; rather a variety of assets are always discussed with different investors becoming part of different ticker discussions. 

%\paragraph{Sensitivity of Contagion Dynamics to $A_0$}

%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=\textwidth]{Figures/VAB/A0_sensitivity.pdf}
%    \caption{\textbf{Sensitivity of Investor Dynamics to $A_0$}; this plot shows that the dynamics are relatively insensitive to how we initialize $A_0$. }
%    \label{fig:A0_sens}
%\end{figure}

%We also consider how dynamics develop for different choices of $A_0$, the number of initial investors who become interested and spread interest in an asset, and plot the evolution for two different values of $A_0$ in Figure \ref{fig:A0_sens} while keeping all other parameters constant. The model appears relatively insensitive to this parameter. A change of $A_0$ from 80 to 10,000 drives only a modest change in the evolution of aggregate investor interest. Interest spreads faster in the latter, however, $\text{max}(A)$ appears relatively consistent demonstrating that other parameters contribute more significantly to $\text{max}(A)$ and the overall dynamics. The graph with $A_0$ highlights a potential flaw with the model; when the right epidemic conditions are met, even a small number of $active$ individuals can trigger a large surge of interest. However, our parameters are extracted from a ticker and time when social contagion in $TSLA$ does occur. The spread of interest is not a given for all initialization parameters and, in fact, is relatively rare. 

%\paragraph{Sensitivity of Contagion Dynamics to $N_0$}

%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=\textwidth]{Figures/VAB/N0_sensitivity.pdf}
%    \caption{\textbf{Sensitivity of Investor Dynamics to $N_0$}; this plot shows that the dynamics are highly sensitive to how we initialize $N_0$. A larger $N_0$ results in a disproportionate increase in $\text{max}(A_0)$ and a fast development of the dynamics. }
%    \label{fig:N0_sens}
%\end{figure}

%In WSB, we have a changing population (which we alter in our initialization for the model presented in Figure \ref{fig:VAB_model_applied}). We observe how dynamics develop for a different $N_0$, while keeping all other parameters constants, in Figure  \ref{fig:N0_sens}. Our model appears highly sensitive to this parameter. Even though in the end, the interest spreads to a total number of investors that is proportional to the increase in $N_0$ (this is observed in the final number of \textit{bored} individuals), the interest spreads much quickly for a large $N_0$. This is particularly important as this is tied to a larger $\text{max}(A)$ and a larger potential market impact generated by the discussion.

\clearpage

==> Cells/1_Proposition.tex <==
\begin{proposition}
\label{proposition:strategic_interactions}
    
    If expressed sentiments are complementary, then the value of additional information is increasing in the information acquisition of other investors.
    
\end{proposition}

\begin{proof}
    
    See Proposition 1 by \citet{hellwig2009knowing}.
    
\end{proof}

==> Cells/2_Definition.tex <==
\begin{definition}
\label{definition:hype_investor_demand}
    
    Hype investor demand $Y_t$ is composed of i) the average buying/selling intensity across all active hype investors, $\phi_t \in [0,1]$, ii) the average purchasing power by hype investor $M/p_t$, and  iii) the total number of hype investors $N$:
    \begin{align}
        p_tY_{t} = MN \phi_{t}.
    \end{align}
    
\end{definition}


==> Cells/3_Assumption.tex <==
\begin{assumption}
\label{assumption:other_investors}
    
    Non-hype investors keep the nominal value invested in the asset fixed, $\Delta (p_tS_t) = 0$.
    
\end{assumption}

==> Cells/3_Proposition.tex <==
\begin{proposition}
\label{proposition:ret}
    
    A uniform, marginal increase (decrease) in an asset's returns will raise (lower) the future outlook of an investor about the asset. It will also indirectly increase (decrease) the outlook of an investor through increasing (decreasing) the outlook of his peers.
    
\end{proposition}

==> Cells/4_Proposition.tex <==
\begin{proposition}
\label{proposition:vol}
    
    If $g(\cdot)$ is decreasing in stock volatility, a uniform, marginal increase in an asset's volatility will directly decrease the future outlook of an investor about the asset. It will also indirectly decrease outlook of an investor through decreasing the outlook of his peers.
    
\end{proposition}

\begin{proof}
    
    Follows from the assumption that $g(\cdot)$ is monotonic and continuous.
    
\end{proof}

==> Cells/5_Assumption.tex <==
\begin{assumption}
\label{assumption:capacity}
    
    Capacity $C = MN/p_tQ$ remains fixed.
    
\end{assumption}

==> Cells/5_Proposition.tex <==
\begin{proposition}
\label{proposition:discrete_time_returns}
    
    Given Eq. \ref{eq:hype_demand} for hype investor demand, and Assumption \ref{assumption:other_investors} for non-hype investor demand, asset price returns can be modeled as:
    
    \begin{align}
        r_{t+1} =  \underbrace{\frac{MN}{p_t Q}}_{\text{(1)\ Capacity}} \times \underbrace{ \Delta \phi_{t+1}}_{\text{(2)\ Demand}}.
        \label{eq:full_price_dynamic_explained}
    \end{align}
    
\end{proposition}

\begin{proof}
    
    Eq. \ref{eq:full_price_dynamic_explained} follows from the first difference of the market capitalization:
    \begin{align}
        \Delta (p_{t+1} Q) = \Delta (p_{t+1} Y_{t+1}) + \Delta (p_{t+1} S_{t+1}) = MN \Delta \phi_{t+1},
    \end{align}
    where equality holds because $\Delta (p_{t+1} S_{t+1}) = 0$ by Assumption \ref{assumption:other_investors}, and Eq. \ref{eq:hype_demand} for $p_{t+1}Y_{t+1}$. Rearranging, and substituting $r_{t+1} = \Delta p_{t+1}/p_t$ yields the desired result.
    
\end{proof}

==> Cells/6_Assumption.tex <==
\begin{assumption}
\label{assumption:extreme_value}
    
    $\epsilon_{i}^+$ is independent and identically distributed, following a type-I Extreme Value (EV) distribution. The same holds for $\epsilon_{i}^-$.
    
\end{assumption}

==> Cells/6_Proposition.tex <==
\begin{proposition}
\label{proposition:discrete_time_sentiments}
    
    The average buying intensity across $N$ hype investors is
    
    \begin{align}
    \label{eq:aggregate_buying_intensity}
        \phi_{t+1} &= \text{tanh}\left[ \frac{\beta r_t + \alpha \phi_{t}}{\lambda}\right].
    \end{align}
    
\end{proposition}

\begin{proof}
    
    Aggregate buying intensity $\phi_{t+1}$ follows from Eq. \ref{eq:phi_probability};
    \begin{align*}
        \phi_{t+1} = \frac{1}{N} \sum^N_{i=1} \text{P}(\phi_{i,t+1}^D = +1) - \text{P}(\phi_{i,t+1}^D = -1) = \frac{\text{exp}\left[( \alpha{\phi}_{t} + \beta r_t)/\lambda\right] - 1}{\text{exp}\left[( \alpha{\phi}_{t} + \beta r_t)/\lambda\right] + 1} = \text{tanh}\left[ \frac{\beta r_t + \alpha \phi_{t}}{\lambda}\right].
    \end{align*}
    
\end{proof}

==> Figures/Consensus/Networks/network_diagram.tex <==
\begin{figure}[!ht]

\begin{center}
\begin{tikzpicture}[->, >=stealth, ultra thick]
    
    \node (author_1) [full_node] {1};
    \node (post_1) [post_node, right of = author_1, xshift = 4cm] {A};
    
    \node (author_2) [full_node, below of = author_1, yshift = -0.1cm] {2};
    
    \node (author_3) [full_node, below of = author_2, yshift = -0.1cm] {3};
    \node (post_2) [post_node, right of = author_3, xshift = 4cm] {B};
    
    \node (author_4) [full_node, below of = author_3, yshift = -0.1cm, dashed] {4};
    
    \node (author_5) [full_node, below of = author_4, yshift = -0.1cm] {5};
    \node (post_3) [post_node, right of = author_5, xshift = 4cm] {C};
    
    \node (author_6) [full_node, below of = author_5, yshift = -0.1cm] {6};
    
    \draw (author_1) to node[above, pos = 0.4]{author} (post_1) ;
    \draw (post_1) to (author_2) [dashed];
    \draw (post_1) to node[above, sloped, pos = 0.6]{comment} (author_3) [dashed];
    
    \draw (author_3) to (post_2);
    \draw (post_2) to node[above, sloped, pos = 0.6]{read?} (author_4) [dotted];
    \draw (post_2) to (author_5) [dotted];
    
    \draw (author_5) to (post_3);
    \draw (post_3) to (author_6) [dashed];
    
    \node (ghost_1) [right of = post_1] {};
    \node (ghost_2) [right of = post_3, yshift = -1.5cm] {};
    \draw (ghost_1) to node[above, sloped]{time} (ghost_2);
    
    \node [left of = author_4, xshift = -1.75cm]{
    \begin{minipage}{4cm}
        User features: 
        \begin{itemize}
        \setlength\itemsep{-0.5em}
            \item External activity,
            \item Active time,
            \item Account age,
            \item Total score.
        \end{itemize}
        Submission features: 
        \begin{itemize}
        \setlength\itemsep{-0.5em}
            \vspace{-0.35cm}\item Score (upvotes),
            \item Comment count,
            \item Ticker extract,
            \item Sentiment,
            \item Topic.
        \end{itemize}
    \end{minipage}
    };
    
    \node (tag_1) [below of = author_6] {$\underbrace{   }_{\text{\large Users}}$};
    \node (tag_2) [right of = tag_1, xshift = 1.5cm] {$\underbrace{\qquad \qquad \qquad}_{\text{\large Interactions}}$};
    \node (tag_3) [right of = tag_2, xshift = 1.5cm] {$\underbrace{   }_{\text{\large Submissions}}$};

\end{tikzpicture}    
\end{center}

    \caption{\textbf{Diagramatic representation of user interactions on WSB}; we encode how information on a specific asset propagates through WSB in a bipartite graph, with submissions on the right and users on the left. Dotted edges represent possible \textit{read} interactions; a dashed line shows if the author comments on the submission. Solid edges denote users authoring submissions. Some of the relevant metadata available for each node type is listed on the left. Only users who author, or comment, on a submission are observed. Other users may not visibly interact with WSB content, but perhaps are exposed to it due to the time they are active on the forum, such as user \textbf{4}.}
    \label{fig:network_diagram}
\end{figure}


==> Figures/Consensus/Networks/network_diagram2.tex <==
\begin{figure}[!ht]

\begin{center}
\begin{tikzpicture}[->, >=stealth, ultra thick]

    \node (author_1) [full_node] {1};
    \node (post_1) [post_node, right of = author_1, xshift = 4cm] {A};
    
    \node (author_2) [full_node, below of = author_1, yshift = -0.1cm] {2};
    \node (post_2) [post_node, right of = author_2, xshift = 4cm] {B};
    
    \node (author_3) [full_node, below of = author_2, yshift = -0.1cm] {3};
    \node (post_3) [post_node, right of = author_3, xshift = 4cm] {C};
    
    \node (author_4) [full_node, below of = author_3, yshift = -0.1cm] {4};
    \node (post_4) [post_node, right of = author_4, xshift = 4cm] {D};
    \node (post_5) [post_node, below of = post_4, yshift = -0.1cm] {E};

    \draw (author_1) to node[above, pos = 0.4]{author} (post_1);
    \draw (author_2) to (post_2);
    \draw (author_3) to (post_3);
    \draw (author_4) to (post_4);
    \draw (author_4) to (post_5);
    
    
    \draw (post_1) to (author_3) [dashed];
    \draw (post_2) to (author_3) [dashed];
    \draw (post_3) to node[above, sloped, pos = 0.6]{comment} (author_4) [dashed];
    
    \node (ghost_1) [right of = post_1] {};
    \node (ghost_2) [right of = post_5] {};
    \draw (ghost_1) to node[above, sloped]{time} (ghost_2);
    
    \node (tag_1) [below of = post_5] {$\underbrace{   }_{\text{\large Submissions}}$};
    \node (tag_2) [left of = tag_1, xshift = -1.5cm] {$\underbrace{\qquad \qquad \qquad}_{\text{\large Interactions}}$};
    \node (tag_3) [left of = tag_2, xshift = -1.5cm] {$\underbrace{   }_{\text{\large Users}}$};
    %\node (tag_2) [right of = tag_1, xshift = 1.5cm] {$\underbrace{\qquad \qquad \qquad}_{\text{\large Interactions}}$};

\end{tikzpicture}    
\end{center}

    \caption{\textbf{Diagramatic representation of user interactions on WSB}; over time,.}
    \label{fig:network_diagram2a}
\end{figure}

==> Figures/Consensus/Networks/network_diagram3.tex <==
\begin{figure}[!ht]

\begin{center}
\begin{tikzpicture}[->, >=stealth, ultra thick]
    
    \node (post_1) [post_node] {A};
    \node (post_2) [post_node, below of = post_1, yshift = -1cm] {B};
    \node (post_3) [post_node, right of = post_2, xshift = 1cm] {C};
    \node (post_4) [post_node, right of = post_3, xshift = 1cm] {D};
    \node (post_5) [post_node, above of = post_4, yshift = 1cm] {E};
    
    \draw (post_1) to (post_3) ;
    \draw (post_2) to (post_3) ;
    \draw (post_3) to (post_4) ;
    \draw (post_3) to (post_5) ;

    \node (tag_1) [below of = post_2] {$\underbrace{   }_{\text{\large IV}}$};
    \node (tag_2) [right of = tag_1, xshift = 1cm] {$\underbrace{\qquad \qquad \qquad}_{ \Bar{\Phi}_{-i,j,(t-1)}}$};
    \node (tag_3) [right of = tag_2, xshift = 1cm] {$\underbrace{   }_{\Phi_{i,j,t}}$};
    
    \node (ghost_1) [below of = tag_1] {};
    \node (ghost_2) [below of = tag_3] {};
    \draw (ghost_1) to node[above, sloped]{time} (ghost_2);
    
\end{tikzpicture}    
\end{center}

    \caption{\textbf{Diagramatic representation of user interactions on WSB}; over time,.}
    \label{fig:network_diagram2b}
\end{figure}

==> Sections/3_Model_old.tex <==
\section{Social dynamics and asset prices}
\label{sec:model}

What motivates investors to share trading advice online? Some seasoned traders might argue that one can only have an investment edge while others are unaware of your strategy. We rationalize our observed online interactions through an asset demand model by incorporating information complementarities in investment decisions. This gives rise to \textit{social contagion} in asset demand; investors buy the asset because others do as well, irrespective of their personal beliefs. The model explores the patterns of returns when this behaviour is present. %If significant, can create reversals in asset price returns. 

Our proposed mechanism is motivated by a growing literature on strategic information complementarities \citep{hellwig2009knowing,zenou2016key}, as well as studies of diagnostic expectations \citep{bordalo2021diagnostic}. Investors trade on the momentum of the stock price, against a supply of shares provided by noise traders.  Our inclusion of a social component subsequently induces persistence in asset demand over time, which leads to reversal in future returns.

\subsection{General setup}
\label{subsec:asset_demand}
We analyse price for one asset traded by $N$ investors, indexed by $i$. Each investor derives CARA utility from consuming $c$, $U_i(c_i) = -\text{exp}(-\gamma c_i)$, where $\gamma$ is the constant absolute rate of risk aversion. We do not include any discounting in their decision-making, but assume they evaluate an asset according to a log-normal distributed value $v = \log(V)$ with expectation $\mathbb{E}_i(v)$ and variance $\sigma^2_i(v)$.

To build intuition, we drop the time subscript and initially present a static version of the model. Investor $i$ purchases $\phi_i$ shares at the current market log-price $p$ to optimise the mean-variance objective function \begin{align}
\label{eq:mean_variance_tradeoff}
    \mathcal{L}(\phi_i) &= [\mathbb{E}_i(v) - p]\phi_i - \frac{\gamma}{2}\sigma^2_i(v)\phi_i^2, \\
    \Rightarrow \phi_i^\ast &= \frac{\mathbb{E}_i(v) - p}{\gamma \sigma^2_i(v)}, \label{eq:optimal_demand}
\end{align}
where an asterisk denotes the value that maximises objective $\mathcal{L}$. In this way, we distinguish between beliefs about value $\mathbb{E}_i(v)$ from investor $i$'s decision to buy amount $\phi_i$. Eq. \ref{eq:optimal_demand} yields a familiar expression for asset demand in equilibrium: namely a ratio of expected net returns over their variance.

\paragraph{Simple price equilibrium} We assume that asset supply originates from noise traders, as in \citet{bordalo2021diagnostic}, to find a price equilibrium. In effect, equilibrium demands sum to exogenous supply $S$: 
\[
\sum^N_{i=1} \phi_i^\ast= S.
\]
Assuming common variance $\sigma^2 = \sigma^2_i(v)$ and averaging expected values $\mathbb{E}(v) = {1}/{N} \sum \mathbb{E}_i(v)$, we can re-arrange Eq. \ref{eq:optimal_demand} to yield the following expression for the market-clearing price $p$:
\begin{align}
    p = \mathbb{E}(v) - \frac{S}{N} \gamma \sigma^2. \label{eq:simple_equilibrium}
\end{align}
Eq. \ref{eq:simple_equilibrium} accounts for the price level by investor's average expected value of the asset, in addition to their ability to absorb the exogenous level of assets supplied. This ability depends on the depth of the investor pool -- reflected by the number of investors $N$ -- as well as their risk appetite $\gamma \sigma^2$. In this simple market, the price increases with expected value, and decreases with supply.

\paragraph{Goals} The first goal of this section is to demonstrate the extent to which asset demand between investors is a strategic complement. The model we consider imposes no cost on investors' information acquisition, which means they anticipate the price of the asset to be high when asset demand by other investors is high. A long literature investigates the link between subjective asset price beliefs and prices, and our contribution will be to introduce a term for social learning. 

The current expression for price ignores heterogeneity and aggregation. Eq. \ref{eq:simple_equilibrium} mimics a single representative investor of some size $N$. However, strategic interactions may give rise to feedback loops in investor demands that do not average out. We extend the model to consider investor heterogeneity. Investors central in a social network are `indirectly' large by their ability to sway others. We make use of this in our empirical study in Section \ref{sec:market_impact}.

The final goal is to investigate the equilibrium price in a dynamic setting where investors are influenced not only by information from peers, but also by other psychological factors - namely extrapolation \citep{glaeser2017extrapolative}. The model produces several predictions about the behaviour of asset prices in the presence of such investors, which we empirically validate later in the paper. We highlight the empirical challenge in a scenario where investor sentiments respond to real-time market events, but point out that the persistence of a social signal may produce variation in asset demand orthogonal to current returns. We use this fact in Section \ref{sec:market_impact} to gauge the extent WSB users exert market impact.

\subsection{Static model with investment complementarities} 

% \paragraph{Payoff under uncertainty} The first stage of this model corresponds to the information acquisition problem studied by \citet{hellwig2009knowing}. Investor $i$'s maximised payoff from Eq. \ref{eq:mean_variance_tradeoff} is
% \begin{align}
%     \mathcal{L}(\phi_i^\ast) &= \frac{1}{2\gamma} \frac{\mathbb{E}_i^2(v-p)}{\mathbb{E}_i(v-p)^2} \label{eq:optimal_payoff} \\
%     % &= \frac{1}{2\gamma} \left(1 - \frac{\mathbb{E}_i[\mathbb{E}_i(v) - v]^2}{\mathbb{E}_i(v-p)^2}\right),
%     &= \frac{1}{2\gamma} \left(1 - \frac{\sigma_i^2(v-p)}{\mathbb{E}_i(v-p)^2}\right),    
% \end{align}
% where the term $\sigma_i^2$ denotes investors' variance for expected return $\sigma_i^2(v-p) = \mathbb{E}_i(v-p)^2 - \mathbb{E}_i^2(v-p)$. At this optimised level, payoffs decrease as uncertainty about return $v-p$ increases, to the extent that squared returns themselves are low. This expression demonstrates the value of social networking. If investors start with different signals about the asset's value, the ability to aggregate them by coordinating with others improves the precision of their expectation, and their final expected payoff. Investors benefit from a better estimate of value $v$ at any price $p$.

% The significance of price and expected value deviations $\mathbb{E}_i(v-p)^2$ remains unclear. Since asset supply, and consequently price, is not revealed, investors are asked to choose information based on their expectation of price. Looking at Eq. \ref{eq:simple_equilibrium}, investors expect the price to be a realisation of aggregated expected value and a mean zero, unobserved supply shock $S$. The difficulty in solving for the market-clearing price lies in the non-linear aggregation of demand. Price is not linear in the expectations of value, nor in the uncertainty faced by individuals.

% We further simplify the problem by assuming a specific form for investors' price uncertainty:
% \begin{align}
%     \mathbb{E}_i(v - p)^2 = \sigma_i^2(v) + \sigma_i^2(s), \label{eq:price_uncertainty}
% \end{align}
% where $\sigma_i^2(s)$ reflects the variance of supply shock $s = S \gamma \sigma^2 /N$ in Eq. \ref{eq:simple_equilibrium}. This form for uncertainty corresponds to an investor who bases their price expectations on a form on simple equilibrium in Eq. \ref{eq:simple_equilibrium}, but uses their personal expectations and uncertainty to forecast price in the second stage. In addition, expected supply shock $\mathbb{E}_i(s)$ is assumed to be zero. Further knowledge of other investors' expectations and uncertainties would yield a refined estimate, but work not shown here demonstrates that this expression holds when the first and second moments in expected value are uncorrelated. 

We study the role of complementary investment decisions. To that end, the model operates in two stages. In the first stage, investors build their expectation for the asset's value, using observed signals from their peers and their expectation of the market-clearing price as a function of the expected, and as of yet hidden, supply shock. In the second stage, the asset supply shock is revealed, and investors execute their trades according to their demand curve. 

Let us consider an investor $i$ who expects value $\mathbb{E}_i(v)$ and understands the price setting mechanism. Investor $i$'s maximised payoff from Eq. \ref{eq:mean_variance_tradeoff} is
\begin{align}
    \mathcal{L}(\phi_i^\ast) &= \frac{\mathbb{E}_i^2(v-p)}{2\gamma \mathbb{E}_i(v-p)^2} \label{eq:optimal_payoff} \\
    % &= \frac{1}{2\gamma} \left(1 - \frac{\mathbb{E}_i[\mathbb{E}_i(v) - v]^2}{\mathbb{E}_i(v-p)^2}\right),
    &= \frac{1}{2} \mathbb{E}_i(v - p) \phi^\ast_i  \\
    &= \frac{1}{2} [\mathbb{E}_i(v) - \mathbb{E}(v)]\phi^\ast_i + \frac{\gamma \sigma^2}{2}  \left( \frac{1}{N} \sum_j^N \phi_j^\ast \right) \phi^\ast_i, \label{eq:payoff_complementarity}
\end{align}
where $\mathbb{E}(v) = {1}/{N} \sum \mathbb{E}_i(v)$ as before. Here, investors base their price expectations on the simple equilibrium in Eq. \ref{eq:simple_equilibrium}, but use their personal expectations and constant uncertainty $\sigma^2$ to forecast price in the second stage.

Eq. \ref{eq:payoff_complementarity} demonstrates that the investor's payoff depends on their peers in two regards. First, payoffs increase to the degree that the investor in question expects to outperform others, in terms of the value they realise in the asset. This is seen in the first component, by which buying(selling) the asset increases the payoff to the extent that $i$'s expected value $\mathbb{E}_i(v)$ is higher(lower) than that of their peers. Second, the payoff increase by the average optimal asset demand of all investors in the economy.

\paragraph{Complementarity in asset demand} This asset demand model predicts that social interactions -- knowledge of other's asset purchases -- is a significant component of investors' welfare \textit{in expectation}. Eq. \ref{eq:payoff_complementarity} is a well-known formulation for strategic interactions between agents acting under quadratic loss \citep{zenou2016key}. Deriving Eq. \ref{eq:payoff_complementarity} with respect to two investors' demands reveals their strategic complementarity:
\begin{align}
    \frac{d^2\mathcal{L}(\phi_i^\ast)}{d\phi_j^\ast d\phi^\ast_i} = \frac{\gamma \sigma^2}{2N} > 0. \label{eq:strategic_complementarity}
\end{align}
The emergence of strategic complementarities is due to a crowding effect that investors have on price. The higher asset demand by other investors, the higher the realised price will turn out to be. Before the value of the asset is revealed, investors are motivated to gauge demand by others to better estimate what the price will be, in excess of their personal valuation.

The unweighted average of peer sentiment in Eq. \ref{eq:payoff_complementarity} emerges because we did not provide a specific mechanism by which information about asset demand is transmitted. The acquisition of information under some cost to the investor is an interesting extension, although already studied by \citet{hellwig2009knowing}. Their study offers more rigorous insight into the manifestation of strategic complementarities, as well as the emergence of multiple equilibria, when investors seek to learn about the underlying price from a set of possible signals. 

\paragraph{Aggregating heterogeneous demand}

An investor's demand may have some idiosyncratic preference which is not captured by common factors. For example, an investor may place particular confidence in products he enjoys using, or admire the corporate strategy of certain company leaders. Such sentiments would manifest as idiosyncratic, heterogeneous investor demand. 
    
We re-write Eq. \ref{eq:optimal_demand} to incorporate some unexplained variation in the beliefs of investor $i$:
\begin{align}
    \phi_i^\ast &= \frac{\mathbb{E}_i(v) - p + e_i}{\gamma \sigma^2}, \\
    \Rightarrow p &= \mathbb{E}(v) - \frac{S}{N} \gamma \sigma^2 + \frac{1}{N} \sum_{i=1}^N e_{i},
\end{align}
where $e_i$ is the idiosyncratic component of $i$' asset demand. Consistently with our earlier exercise, investors use personal expectations and constant uncertainty $\sigma^2$ to forecast price. This generalises the price equilibrium in Eq. \ref{eq:simple_equilibrium} to include the average idiosyncratic sentiment shocks of all investors. Under the assumption that these shocks have a finite variance and mean zero, they should average out to zero by the Central Limit Theorem.

\paragraph{Granular shocks} The choice to include idiosyncratic shocks appears to be a trivial extension of the model when the valuations of all investors are weighted equally. However, consider a scenario where some investors have different levels of importance $s_i$ for aggregate demand:
\begin{align}
    S &= \sum_{i=1}^N s_i \phi_i^\ast, \\
    \Rightarrow p &= \sum_{i=1}^N s_i \mathbb{E}_i(v) - \gamma \sigma^2 S + \sum_{i=1}^N s_i e_{i},
\label{eq:granular_social1}
\end{align}
where weights $\sum_i s_i = 1$ for demand to equal supply. This could be the case for several reasons: investors could have different amount of capital or, of greater interest to this paper, some investors may have \textit{more sway} in forming public opinion than others. The importance of key players in a social context has been explored in several economic settings -- see \cite{zenou2016key} for a thorough overview. Typically, the most central nodes in a social network have the ability to quickly diffuse information and, therefore, have a high influence on others. 
    
We justify this weighting scheme by the fact that certain users on WSB have a disproportionate effect in shaping the broader discourse. Indeed, WSB is structured to promote viral content, and we would expected a consensus to be formed by key players -- or, rather, around key submissions. If the distribution of importance does not have a finite variance -- i.e. it is `heavy-tailed' -- then the idiosyncratic shocks would not average out to zero. 

\subsection{Price dynamics with peer effects} 

To study the joint dynamics of an asset's price and demand by social investors, we treat aggregate asset demand $\phi = \sum_i \phi_i$ and log price $p$ as state variables for a dynamic system, indexed by time $t$. In doing so, we assume that cumulative demand $\phi_{t}$ reflects a difference between individual valuations of the asset and the price. We distinguish between two independent components of individual valuations: the private signal of individuals $g(b_{i,t})$ and the signal individuals draw from observations of peers $f(\phi_{i,t})$. Aggregate asset demand and price are
\begin{align}
    \phi_t &= \frac{\mathbb{E}_t[g(b_{i,t})] + \mathbb{E}_t[f( \phi_{i,t})] - p_t}{\gamma \sigma^2}, \label{eq:demand_system} \\
    p_t &= \mathbb{E}_t[g(b_{i,t})] + \mathbb{E}_t[f( \phi_{i,t})] - \frac{S_t}{N}\gamma \sigma^2. \label{eq:price_system}
\end{align}
Cumulative demand is, therefore, the difference between individual valuations and the market-clearing price, normalized by risk-aversion. The market-clearing price, on the other hand, is the difference between individual valuations and the rate of asset supply, normalized by the number of investors $N$ and their risk appetite $\gamma\sigma^2$, similar to Eq. \ref{eq:simple_equilibrium}. 

A focus of this paper is the relationship between valuations $g(b_{i,t})$ and the social component $f(\phi_{i,t})$. Studies in behavioural finance suggest different expectation formation mechanisms that ultimately deviate from rational expectations \citep{barberis2018extrapolation,bordalo2021diagnostic}. We combine two such features in Assumptions \ref{assumption:complementarity} and \ref{assumption:mech_extrapolation} to propose a testable structure for $\mathbb{E}_t[f(\phi_{i,t})]$ and $\mathbb{E}_t[g(b_{i,t})]$.

\paragraph{Persistent demand} The mechanism by which past demand enters current asset demand is by the complementarity in investor payoffs. Investor $i$'s payoff to holding the asset is assumed to increase linearly in average asset demand by others.

\input{Cells/1_Assumption.tex}

Assumption \ref{assumption:complementarity} is in line with the finding that our asset demand model produces strategic complementarities in investor asset demands in Eq. \ref{eq:strategic_complementarity}. Several extensions of the simple formulation are possible to account for greater complexities in social interactions. It can, for example, be extended to take into account \textit{key players} \citep{zenou2016key} through changing the way that people weight the demand of others $\phi_{i,t-1}$ in the sum $1/N \sum_i \phi_{i,t-1}$ to $\sum_i s_i \phi_{i,t-1}$, where $s_i$ captures the influence of player $i$ and $\sum_i s_i = 1$. 

In more complex settings, we can consider the unique complementarities between connected individuals as described in \cite{zenou2016key}, clusters of investors \citep{bouchaud2003theory}, or alternative information spreading / individual targeting models, which have received attention in the recent literature \citep{galeotti2020targeting}. The added complexity would affect aggregate demand through the expectations of other's demand $\phi_{t-1}$.

\paragraph{Mechanical Extrapolation} We assume that investors partially trade on the momentum of the asset's price, which \citet{bordalo2021diagnostic} term `mechanical extrapolation'. The functional form of $\mathbb{E}_t[g(b_i)]$ is specified in Assumption \ref{assumption:mech_extrapolation}.

\input{Cells/1.1_Assumption}

Mechanical extrapolation is our preferred way to introduce a relationship between prices and demand \citep{barberis2018extrapolation}. A model with mechanical extrapolation has several shortcomings, one of which is the inability to relate expectation updates to psychological underpinnings. However, our assumption is justified by our empirical work in Section \ref{sec:consensus_results} which demonstrates that individuals update their outlook based on recent asset returns. 

\paragraph{System for price and demand} Combining Assumptions \ref{assumption:complementarity} and \ref{assumption:mech_extrapolation} into Eqs. \ref{eq:demand_system}-\ref{eq:price_system} yields demands and returns $r_t = p_t - p_{t-1}$:
\begin{align}
    \phi_t &= \frac{\alpha \phi_{t-1} + \beta r_t}{\gamma \sigma^2}, 
    \label{eq:model_sentiment_return1}
\end{align}
\begin{align}
    r_t &= -\frac{\alpha}{\beta} \phi_{t-1} + \frac{S_t\gamma \sigma^2}{\beta N}.
\end{align}
In this scenario, asset demand and returns are determined simultaneously. The first mechanism is through market clearing, where demand has to adjust to supply. The second is the adjustment of the expected value for the asset to the realised return through $\beta$ and the social signal through $\alpha$. 

As a result, returns are accounted for by current and past asset demand:
\begin{align}
\label{eq:return_against_demand}
    r_t = \frac{\gamma\sigma^2 }{\beta} \phi_t - \frac{\alpha}{\beta} \phi_{t-1},
\end{align}
since supply must equal demand at time $t$. This equation uncovers several important mechanisms at play. Returns are related positively to current demand $\phi_{t}$ through market clearing -- supply $S$ is exogenous and must meet current demand. Higher demand drives up returns. Returns are, however, negatively related to past demand $\phi_{t-1}$ through the expected value of an asset -- a \textit{valuation mechanism}. If there is a positive social signal, investors still value an asset highly, even in the presence of low returns. 

To explain the basic intuition, we consider the following scenarios: i) one where the asset has a positive return $r_t$ and no social signal $\phi_{t-1}$, and ii) one where investors observe a positive social signal $\phi_{t-1}$. In scenario (i), demand is driven by the extrapolation component alone -- investors believe that returns will continue to increase based on the current trend. In scenario (ii) on the other hand, investors do not require a large return to demand the asset -- positive past sentiment drives current demand $\phi_t$. Under exogenous supply, a strong positive signal from peers means that the extrapolated return is \textit{less} important in justifying a higher price. The underlying reasoning relies on the fact that the system is in equilibrium. Therefore, both returns and sentiments have adjusted to reflect a new steady-state, where sentiments are at a certain level $\phi_t$. %It is also, implicitly, not the correct setting to study granular social shocks and their aftermath.

Finally, we observe that the ratios of the coefficients, $\gamma/\beta$ and $\alpha/\beta$, play an important role. $\beta$ effectively anchors the demand of investors in reality -- a greater value of $\beta$ implies that social signals carry less weight, and investors focus on price trends to forecast and expect asset values to grow at some constant rate. As $\beta$ decreases, returns are determined more by social forces -- hype from peers, rather than past performance, now justifies returns and demand. In our data, we observe that $\beta$ is roughly five times $\alpha$ -- individuals weight the sentiments of peers, however, returns are necessary to justify their investment strategies. $\sigma^2$ serves to taper the impact of sentiment, since investors are less certain in their signal and demand less of the asset.

\paragraph{Persistent fluctuations} The reversal in returns is an important feature that emerges from social contagion in investors' price expectations. If large enough, these can produce bubbles in asset prices: initial momentum from positive news creates a price run-up, before an absence of news creates a drought of new asset demand. The subsequent price crash carries on its own momentum. We can treat demand as a latent variable to see these oscillations manifest in return data. Substituting lagged demand into the equation for returns, and iterating infinitely yields
\begin{align}
\label{eq:return_time_series}
    r_t = -\sum_{T = 1}^\infty \left(\frac{\alpha}{\gamma \sigma^2}\right)^T r_{t-T} + \frac{S_t\gamma \sigma^2}{\beta N}
\end{align}
as long as $\alpha / \gamma \sigma^2 < 1$, so that the contribution of demand fluctuations to returns converges to zero over time. This is an autoregressive model with infinite lags, where the coefficients decrease exponentially with lag size $T$. Without any knowledge of asset demand, the second term encapsulates an unobservable error term, which the model links to exogenous changes in the asset's supply. Eq. \ref{eq:return_time_series} demonstrates that an exogenous increase in returns at time $t$ is followed by a smaller decrease in $t+1$. This oscillation persists indefinitely, and would converge to zero rapidly if the social signal $\alpha / \gamma \sigma^2$ is sufficiently small.

\subsection{Model predictions}

A simple linear regression exercise in Table \ref{tab:characteristic_regression} provides some evidence of the validity of the model proposed by Eq. \ref{eq:return_against_demand}. We summarise our asset demand model with social contagion by three further predictions, which we seek to validate in our WSB data.

%The R-squared fit is small, since the social investors we sample using WSB constitute a relatively small share of total trading activity.

\paragraph{Prediction 1: A mechanism for peer effects in asset demand} \textit{Given that asset demands by social investors are complementary, a marginal increase(decrease) in peer outlook about an asset will raise(lower) the future outlook of an investor about the asset.}

We dedicate Section \ref{sec:social_dynamics} to investigating strategic complementarities among investors on WSB. Besides testing for the direct effect of peers on investor sentiment (Prediction 1), we also use the opportunity to test our assumption for mechanical extrapolation: A uniform, marginal increase(decrease) in an asset's returns will raise (lower) the future outlook of an investor about the asset. It will also indirectly increase(decrease) the outlook of an investor through increasing(decreasing) the outlook of peers.

\paragraph{Prediction 2: Return predictability} \textit{An increase in asset demand explained by past investor sentiment increases the asset's price.}

According to Eq. \ref{eq:return_against_demand}, there is a positive contemporaneous correlation between returns and WSB sentiments, but a negative correlation with lagged sentiments. However, one issue with the positive correlation is the challenge of identification. The data typically reflects an equilibrium outcome where sentiments and returns are positive, and vice versa. The main challenge is to identify exogenous variations in current sentiment relative to current returns. If current sentiments do not depend on future returns, we can estimate the impact of WSB sentiments on returns using sentiment scores predicted from preceding discussions. Stock-specific characteristics will also drive persistent heterogeneity in the expressed sentiments of WSB users. We tackle the question of whether social dynamics can account for some return predictability in Section \ref{sec:market_impact}.

\paragraph{Prediction 3: Granular social forces} \textit{Idiosyncratic demand shocks do not average out in the presence of heavy-tailed attention and impact asset prices.}

Eq. \ref{eq:granular_social1} predicts that, in the presence of heavy-tailed attention to certain investors, heterogeneity in investor sentiments will not average out, and will instead have an impact on asset prices. An emphasis on viral content compels WSB discussants to follow specific, popular strategies, which are predicted to have an outsized impact on asset price returns. We investigate the role of these granular idiosyncratic sentiments in Section \ref{sec:market_impact}.

==> Tables/Jacobian_SS.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, Jan 18, 2022 - 12:28:08
\begin{table}[!ht]
\begin{center}

\caption{System behaviour around steady states and Jacobian Eigenvalues} 
\label{tab:jacobian_steady_states} 
\begin{tabular}{@{\extracolsep{10pt}}ccc} 

\toprule \\[-1.8ex] 
$|x_i| < 1$ & $\mathbb{I} (x_i)$ = 0 & stable node / sink \\ 
$|x_i| < 1$ & $\mathbb{I} (x_i) \neq$ 0 & stable focus / spiral sink \\ 
$|x_i| > 1$ & $\mathbb{I} (x_i)$ = 0 & unstable node / source \\ 
$|x_i| > 1$ & $\mathbb{I} (x_i) \neq$ 0 & unstable focus / spiral source \\ 

\bottomrule \\[-1.8ex] 
\end{tabular} 
\end{center}
\footnotesize{ \textit{Notes}: The behaviour of our system around our steady states is dependent on the eigenvalues of the Jacobian at the steady states. Here we describe some of the most common eigenvalue combinations and behaviours. For a more comprehensive review, see \cite{hommes2013behavioral}. }

\end{table} 


==> Tables/adjacent_sentiment_spillovers.tex <==
\begin{table}[ht] 

\caption{WSB Sentiment Spillovers} 
\label{tab:adjacent_sentiment_spillovers}
\resizebox{\textwidth}{!}{
    \begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
    \hline \\[-1.8ex] 
     & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
    \cline{2-7} 
    \\[-1.8ex] & $\phi_i = -1$ & $\phi_i = +1$ & $\phi_i = -1$ & $\phi_i = +1$ & $\phi_i = -1$ & $\phi_i = +1$ \\ 
    & (1) & (2) & (3) & (4) & (5) & (6)\\ 
    \hline \\[-1.8ex]
    
    $R^e$ & $-$.46$^{***}$ (.07) & .03 (.03) & $-$.46$^{***}$ (.07) & .02 (.03) & $-$.47$^{***}$ (.07) & .02 (.03) \\ 
    $\widetilde{R^e}$ & $-$.21$^{***}$ (.04) & .04$^{***}$ (.02) & $-$.20$^{***}$ (.04) & .04$^{***}$ (.02) & $-$.19$^{***}$ (.04) & .03$^{**}$ (.02) \\ 
    $\sigma$ & $-$.84$^{***}$ (.16) & $-$.95$^{***}$ (.10) & $-$.86$^{***}$ (.16) & $-$.97$^{***}$ (.10) & $-$.96$^{***}$ (.16) & $-$1.00$^{***}$ (.11) \\ 
    $\phi^+_{-1}$ & $-$.44$^{***}$ (.03) & .45$^{***}$ (.02) & $-$.42$^{***}$ (.03) & .46$^{***}$ (.02) & $-$.43$^{***}$ (.04) & .48$^{***}$ (.02) \\ 
    $\phi^0_{-1}$ & $-$.80$^{***}$ (.03) & $-$.38$^{***}$ (.02) & $-$.78$^{***}$ (.03) & $-$.37$^{***}$ (.02) & $-$.81$^{***}$ (.03) & $-$.39$^{***}$ (.02) \\ 
    $\phi^-_{-1}$ & .72$^{***}$ (.04) & $-$.17$^{***}$ (.04) & .72$^{***}$ (.04) & $-$.16$^{***}$ (.04) & .76$^{***}$ (.04) & $-$.16$^{***}$ (.04) \\ 
    $\phi^{\text{NA}}_{-1}$ & $-$.22$^{***}$ (.02) & .04$^{***}$ (.01) & $-$.23$^{***}$ (.02) & .02 (.01) & $-$.23$^{***}$ (.02) & .03$^{*}$ (.01) \\ 
    $\boldsymbol{W} \boldsymbol{\phi^+}$ &  &  & $-$.12$^{***}$ (.04) & .09$^{***}$ (.03) & $-$.16$^{***}$ (.04) & .08$^{***}$ (.03) \\ 
    $\boldsymbol{W} \boldsymbol{\phi^0}$ &  &  & $-$.21$^{***}$ (.04) & $-$.19$^{***}$ (.03) & $-$.25$^{***}$ (.04) & $-$.19$^{***}$ (.03) \\ 
    $\boldsymbol{W} \boldsymbol{\phi^-}$ &  &  & .39$^{***}$ (.05) & $-$.20$^{***}$ (.05) & .35$^{***}$ (.06) & $-$.19$^{***}$ (.05) \\ 
    $\boldsymbol{W} R^e$ &  &  &  &  & $-$.16 (.20) & .20$^{**}$ (.09) \\ 
    $\boldsymbol{W} \widetilde{R^e}$ &  &  &  &  & $-$.06 (.06) & .02 (.03) \\ 
    $\boldsymbol{W} \sigma$ &  &  &  &  & .93$^{*}$ (.48) & .04 (.36) \\ 
    $m$ & $-$.73$^{***}$ (.01) & $-$.07$^{***}$ (.01) & $-$.71$^{***}$ (.02) & $-$.04$^{***}$ (.01) & $-$.71$^{***}$ (.02) & $-$.04$^{***}$ (.01) \\ 
    
    \hline
    Model & \multicolumn{2}{c}{Baseline} & \multicolumn{2}{c}{Spatial Lag} & \multicolumn{2}{c}{Spatial Durbin} \\
    AIC & \multicolumn{2}{c}{193,749.7} & \multicolumn{2}{c}{193,573.9} & \multicolumn{2}{c}{188,355.5} \\
    McFadden's R\textsuperscript{2} & \multicolumn{2}{c}{.01} & \multicolumn{2}{c}{.01} & \multicolumn{2}{c}{.01} \\
    N & \multicolumn{2}{c}{95,981} & \multicolumn{2}{c}{95,981} & \multicolumn{2}{c}{93,412} \\
    \hline
     & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01}
    \end{tabular}

}
\footnotesize{\textit{Notes:} This table presents estimated log-odds coefficients for three multinomial logit models on the expressed sentiment in WSB submissions. Odd columns estimate the log-odds ratio of submission $i$'s sentiment being bearish, $\phi_i = -1$. Similarly, even columns estimate the ratio of submission $i$'s sentiment being bullish, $\phi_i = +1$. Neutral submissions serve as the benchmark.}
\end{table} 


==> Tables/consensus/old/consensus_2sls.tex <==
\begin{table}[ht!]
\centering
\caption{Peer Influence: Quantifying Peer Influence -- 2SLS Approach}
\begin{tabular}{lcc}
\toprule \toprule
 \multicolumn{3}{l}{\textbf{Panel A: Reduced Form} -- peer influence estimated using the sentiment of posters} \\
  \multicolumn{3}{l}{between an author's posts} \\[1ex]
&  \textit{Independent Variable}  \\ \\[-1.8ex]
&    $\Bar{\phi}_{-i,j,(t-1,t)}$  & Ticker Fixed Effects \\ \cline{2-3} \\[-1.8ex]
Investor Sentiment $(\phi_{i,j,t})$ & 0.11 (0.02) *** &  X \\
\multicolumn{3}{l}{\small{Observations: 11,296, $R^2_{adj}$: 0.07}}\\[2ex]
\toprule
 \multicolumn{3}{l}{\textbf{Panel B: IV} -- peer influence estimated using IV for peer sentiment} \\[1ex]
 &  \textit{Independent Variable} & \\
&  $\Bar{\phi}_{-i,j,(t-1,t)}$  & \\
&  average peer sentiment (predicted)  & Ticker Fixed Effects \\ \cline{2-3} \\[-1.8ex]
Investor Sentiment $(\phi_{i,j,t})$ & 0.16 (0.06) **  & X \\
\multicolumn{3}{l}{\small{Observations: 8,505, Instrument residuals J-statistic: 0.00}}\\[2ex]
\toprule
\multicolumn{3}{l}{\textbf{Panel C: First Stage IV} -- investor sentiment estimated using their historical sentiment} \\[1ex]
&  \textit{Independent Variable}  \\ \\[-1.8ex]
&    $\phi_{i,j,(t-1)}$  & Ticker Fixed Effects \\ \cline{2-3} \\[-1.8ex]
Investor Sentiment $(\phi_{i,j,t})$ & 0.32 (0.01) *** &  None \\
\multicolumn{3}{l}{\small{Observations: 15,652, F-statistic: 1,817}}\\[2ex]
\bottomrule
\end{tabular} \\
\bigskip
\begin{tabular}{cccc}
\multicolumn{4}{l}{%
  \begin{minipage}{17cm}%
    \footnotesize{ \textit{Notes}: The first stage is estimated using all submission data from WSB where we observe an author posting more than one time about a ticker. The second stage is estimated using the average predicted sentiment of peers between an author's posts about the same asset. Ticker-level dummies, asset return and volatility controls, and the intercept are included in the second stage but not shown. Robust standard errors, clustered at the ticker level for Panels A and B, are presented in parentheses. Observations with incomplete market data are dropped. The first stage regression achieves an $R^2 = 0.10$, $R^2_{adj} = 0.10$. The second stage has $R^2 = 0.07$, $R^2_{adj} = 0.05$.\\
*** Significant at 1\% level
** Significant at 5\% level
* Significant at 10\% level}
  \end{minipage}}
\end{tabular}
\label{tab:reg_consensus_2sls}
\end{table}


==> Tables/consensus/old/consensus_full2sls.tex <==
\begin{table}[ht!]
\centering
\caption{Peer Influence: Multiple Posters -- Full Second Stage}
\begin{tabular}{llc}
\toprule \toprule
 && \textit{Dependent Variable}\\
 && $\phi_{i,j,t}$ \\
\toprule
%Intercept              &  -2.22 (0.54) *** \\
\multirow{9}{*}{\rotatebox{90}{\textit{Independent Variables}}}
&$\phi_{i,j,t-1}$  &   0.17 (0.01) *** \\
&$\Bar{\phi}_{-i,j,t-1}$ (estimated)           &    0.16 (0.06) ** \\
& $R_{j,t}$         &   0.93 (0.24) *** \\
&$\Bar{R}_{j,t}$   &      0.51 (0.71)  \\
&$\sigma(R_{j,t})$ &     0.11 (0.67)  \\
&$min_{j,t}$       &    0.80 (0.31) ** \\
& $max_{j,t}$       &    0.59 (0.32) * \\
& $(max-min)_{j,t}$ &    -0.20 (0.22)  \\
&Ticker Fixed Effects & X \\
\bottomrule
\end{tabular} \\
\bigskip
\begin{tabular}{cccc}
\multicolumn{4}{l}{%
  \begin{minipage}{16cm}%
    \footnotesize{ \textit{Notes}: The dependent variable is individual investor sentiment about an asset, scaled continuously between $(-\infty, \infty)$. We estimate it using the individual's previously expressed sentiment about the same asset ($\phi_{i,j,t-1}$) and the sentiment of his peers in the time between his posts ($\Bar{\phi}_{-i,j,(t-1,1)}$), as well as a set of control market variables and ticker-level fixed effects. Robust standard errors, clustered at the ticker level, are presented in parentheses. Observations with incomplete market data are dropped. The sample includes 8,505 observations. The regression achieves an $R^2 = 0.07$, $R^2_{adj} = 0.05$.\\
*** Significant at 1\% level
** Significant at 5\% level
* Significant at 10\% level}
  \end{minipage}}
\end{tabular}
\label{tab:reg_consensus_2nd_stage}
\end{table}


==> Tables/consensus/old/consensus_network.tex <==
\begin{table}[ht!]
\centering
\caption{Peer Influence: Quantifying Peer Influence -- Network Approach}
\begin{tabular}{lcc}
\toprule \toprule
 \multicolumn{3}{l}{\textbf{Panel A: Reduced Form} -- investor sentiment estimated using the sentiment of his neighbours} \\[1ex]
&  \textit{Independent Variable}  \\ \\[-1.8ex]
&    $\Bar{\phi}_{-i,j,(t-1)}$  & Ticker Fixed Effects \\ \cline{2-3} \\[-1.8ex]
Investor Sentiment $(\phi_{i,j,t})$ & 0.07 (0.01) *** &  X \\
\multicolumn{3}{l}{\small{Observations: 19,893, $R^2_{adj}$: 0.05}}\\[2ex]
\toprule
 \multicolumn{3}{l}{\textbf{Panel B: IV} -- peer influence estimated using IV for neighbour sentiment} \\[1ex]
 &  \textit{Independent Variable} & \\
&  $\Bar{\phi}_{-i,j,(t-1)}$  & \\
&  Average Neighbour Sentiment (predicted)  & Ticker Fixed Effects \\ \cline{2-3} \\[-1.8ex]
Investor Sentiment $(\phi_{i,j,t})$ & 0.34 (0.07) ***  & X \\
\multicolumn{3}{l}{\small{Observations: 19,620, Instrument residuals J-statistic: 0.00}}\\[2ex]
\toprule
 \multicolumn{3}{l}{\textbf{Panel C: First Stage IV} -- sentiment of neighbours estimated using neighbour's neighbours} \\[1ex]
&  \textit{Independent Variable}  \\ \\[-1.8ex]
&    Sentiment of Neighbours' Neighbours  & Ticker Fixed Effects \\ \cline{2-3} \\[-1.8ex]
Sentiment of Neighbours & 0.19 (0.01) *** &  None \\
\multicolumn{3}{l}{\small{Observations: 27,630, F-statistic: 655}}\\[2ex]
\bottomrule
\end{tabular} \\
\bigskip
\begin{tabular}{cccc}
\multicolumn{4}{l}{%
  \begin{minipage}{17cm}%
    \footnotesize{ \textit{Notes}: The first stage is estimated using the sentiment of the previous posts that the author of a post has commented on (about the same asset). The second stage is estimated using the average predicted sentiment of posts an author comments on. Ticker-level dummies, asset return and volatility controls, and the intercept are included in the second stage but not shown. Robust standard errors, clustered at the ticker level for Panels A and B, are presented in parentheses. Observations with incomplete market data are dropped. The first stage regression achieves an $R^2 = 0.10$, $R^2_{adj} = 0.10$. The second stage has $R^2 = 0.07$, $R^2_{adj} = 0.05$.\\
*** Significant at 1\% level
** Significant at 5\% level
* Significant at 10\% level}
  \end{minipage}}
\end{tabular}
\label{tab:reg_consensus_network}
\end{table}


==> Tables/consensus/old/consensus_reg.tex <==
\begin{table}[ht!]
\centering
\caption{Peer Influence: Multiple Posters -- Reduced Form Regression Estimates}
\begin{tabular}{llc}
\toprule \toprule
 && \textit{Dependent Variable}\\
 && $\phi_{i,j,t}$ \\
\toprule
%Intercept              &  -2.22 (0.54) *** \\
\multirow{9}{*}{\rotatebox{90}{\textit{Independent Variables}}}
& $\phi_{i,j,t-1}$            &   0.16 (0.01) *** \\
& $\Bar{\phi}_{-i,j,(t-1,t)}$ &   0.11 (0.02) *** \\
& $R_{j,t}$                   &   0.84 (0.16) *** \\
& $\Bar{R}_{j,t}$             &      0.46 (0.62)  \\
& $\sigma(R_{j,t})$           &      0.18 (0.42)  \\
& $min_{j,t}$                 &   0.75 (0.21) *** \\
& $max_{j,t}$                 &    0.39 (0.18) ** \\
& $(max-min)_{j,t}$           &   -0.35 (0.17) ** \\
&Ticker Fixed Effects & X \\
\bottomrule
\end{tabular} \\
\bigskip
\begin{tabular}{cccc}
\multicolumn{4}{l}{%
  \begin{minipage}{16cm}%
    \footnotesize{ \textit{Notes}: The dependent variable is individual investor sentiment about an asset, scaled continuously between $(-\infty, \infty)$. We estimate it using the individual's previously expressed sentiment about the same asset ($\phi_{i,j,t-1}$) and the sentiment of his peers in the time between his posts ($\Bar{\phi}_{-i,j,(t-1,t)}$). Robust standard errors, clustered at the ticker level, are presented in parentheses. Observations with incomplete market data are dropped. The sample includes 11,296 observations. The regression achieves an $R^2 = 0.12$, $R^2_{adj} = 0.07$.\\
*** Significant at 1\% level
** Significant at 5\% level
* Significant at 10\% level}
  \end{minipage}}
\end{tabular}
\label{tab:reg_consensus}
\end{table}


==> Tables/consensus/old/consensus_reg_rand.tex <==
\begin{table}[ht!]
\centering
\caption{Peer Influence: Quantifying Peer Influence -- Random Cohort Test}
\begin{tabular}{llc}
\toprule \toprule
 && \textit{Dependent Variable}\\
 && $\phi_{i,j,t}$ \\
\toprule
\multirow{9}{*}{\rotatebox{90}{\textit{Independent Variables}}}
& $\phi_{i,j,t-1}$            &   0.16 (0.01) *** \\
& $\Bar{\phi}_{-i,j}$ &   -0.01 (0.02) \\
& $R_{j,t}$                   &   0.86 (0.16) *** \\
& $\Bar{R}_{j,t}$             &      0.55 (0.66)  \\
& $\sigma(R_{j,t})$           &      0.14 (0.45)  \\
& $min_{j,t}$                 &   0.76 (0.21) *** \\
& $max_{j,t}$                 &    0.41 (0.18) ** \\
& $(max-min)_{j,t}$           &   -0.35 (0.17) * \\
&Ticker Fixed Effects & X \\
\bottomrule
\end{tabular} \\
\bigskip
\begin{tabular}{cccc}
\multicolumn{4}{l}{%
  \begin{minipage}{16cm}%
    \footnotesize{ \textit{Notes}: The dependent variable is individual investor sentiment about an asset, scaled continuously between $(-\infty, \infty)$. We estimate it using the individual's previously expressed sentiment about the same asset ($\phi_{i,j,t-1}$) and the sentiment of a random cohort of peers who post about the same ticker($\Bar{\phi}_{-i,j}$). Robust standard errors, clustered at the ticker level, are presented in parentheses. Observations with incomplete market data are dropped. The sample includes 11,347 observations. The regression achieves an $R^2 = 0.11$, $R^2_{adj} = 0.07$.\\
*** Significant at 1\% level
** Significant at 5\% level
* Significant at 10\% level}
  \end{minipage}}
\end{tabular}
\label{tab:reg_consensus_rand}
\end{table}

==> Tables/consensus/old/consensus_res_old.tex <==
\begin{table}[ht!]
\centering
\caption{Quantifying Peer Influence}
\begin{tabular}{lcc}
\toprule \toprule
&  \multicolumn{2}{c}{\textit{Independent Variable} -- average peer sentiment, $\Bar{\phi}_{-i,j,(t-1)}$} \\ [1.2ex]
&    Multiple Posters  &  Network \\ 
& (1) & (2) \\
\cline{2-3} \\[-1.8ex]
 \multicolumn{3}{l}{\textbf{Panel A: Reduced Form}} \\
  \multicolumn{3}{l}{\small{Peer influence estimated using observed average sentiment of peers}} \\ [1.2ex]
Investor Sentiment $(\phi_{i,j,t})$ & 0.11 (0.02) ***  &  0.07 (0.01) *** \\
Observations & 11,296 & 19,893\\
$R^2_{adj}$ & 0.07 & 0.05 \\ [2ex]
%\multicolumn{3}{l}{\small{Observations: 19,893, $R^2_{adj}$: 0.05}}\\[2ex]
 \multicolumn{3}{l}{\textbf{Panel B: IV}} \\
  \multicolumn{3}{l}{\small{Peer influence estimated using estimated average sentiment of peers (through IV)}} \\[1.2ex]
Investor Sentiment $(\phi_{i,j,t})$ & 0.16 (0.06) **  & 0.34 (0.07) *** \\
Observations & 8,505 & 19,620 \\
$R^2_{adj}$ & 0.05 & 0.05 \\ 
Instrument residuals J-statistic: & 0.00 & 0.00 \\ [2ex]
\multicolumn{3}{l}{\textbf{Panel C: First Stage IV}}\\
 \multicolumn{3}{l}{\small{Sentiment of peers estimated using instrumental variable}}\\[1.2ex]
&  \multicolumn{2}{c}{\textit{Independent Variable}}  \\
&    Historical Sentiment  & Sentiment of \\ 
&    of Peers   & Neighbours' Neighbours \\ \cline{2-3} \\[-1.8ex]
Sentiment of Peers & 0.32 (0.01) *** &  0.19 (0.01) *** \\
Observations & 15,652 & 27,630\\
$R^2_{adj}$ & 0.10 & 0.10 \\ 
F-statistic: & 1,817 & 655 \\ [2ex]
\bottomrule
\end{tabular} \\
\bigskip
\begin{tabular}{cccc}
\multicolumn{4}{l}{%
  \begin{minipage}{17cm}%
    \footnotesize{ \textit{Notes}: In Column (1), the first stage is estimated using the initial sentiment expressed by an author about an asset to estimate his sentiment in the following post. In Column (2), the first stage is estimated using the sentiment of the previous posts that the author of a post has commented on (about the same asset). The second stage is estimated using the average predicted sentiment of peers. Ticker-level dummies, asset return and volatility controls, and the intercept are included in the second stage and reduced form estimates, but not shown -- the full estimates are presented in Appendix \ref{app:consensus}. Robust standard errors, clustered at the ticker level for Panels A and B, are presented in parentheses. Observations with incomplete data are dropped. \\
*** Significant at 1\% level
** Significant at 5\% level
* Significant at 10\% level}
  \end{minipage}}
\end{tabular}
\label{tab:reg_consensus_main}
\end{table}


==> Tables/consensus/old/hist_max_min.tex <==
\begin{table}[ht!]
\centering
\caption{Relation of Sentiment to Historical Intra-Day Volatility}
\begin{tabular}{lc}
\toprule \toprule
 & \textit{Dependent Variable}\\
 & $\phi_{i,j,t}$ \\
\midrule
$min_{j,t}$                   &   0.69 (0.17) *** \\
$max_{j,t}$                   &   0.34 (0.09) *** \\
$(max-min)_{j,t}$               &  -0.35 (0.09) *** \\
$R_{j,t}$            &   0.34 (0.11) *** \\
$\Bar{R}_{j,t}$ &    1.43 (0.61) ** \\
$\sigma({R}_{j,t})$  &  -0.96 (0.24) *** \\
$min_{j,t-1}$                  &      0.13 (0.12)  \\
$max_{j,t-1}$                  &      0.32 (0.20)  \\
$(max-min)_{j,t-1}$              &     -0.19 (0.17)  \\
$min_{j,t-2}$                  &      0.17 (0.13)  \\
$max_{j,t-2}$               &     0.33 (0.19) * \\
$(max-min)_{j,t-2}$              &     -0.17 (0.16)  \\
$min_{j,t-3}$                  &     -0.16 (0.14)  \\
$max_{j,t-3}$                 &      0.18 (0.19)  \\
$(max-min)_{j,t-3}$             &   -0.35 (0.14) ** \\
$min_{j,t-4}$                 &      0.14 (0.15)  \\
$max_{j,t-4}$                &     0.44 (0.24) * \\
$(max-min)_{j,t-4}$             &    -0.30 (0.16) * \\
Ticker Fixed Effects & X \\
\bottomrule
\end{tabular} \\
\bigskip
\begin{tabular}{cccc}
\multicolumn{4}{l}{%
  \begin{minipage}{16cm}%
    \footnotesize{ \textit{Notes}: The dependent variable is individual investor sentiment, scaled continuously between $(-\infty, \infty)$. Robust standard errors, clustered at the ticker level, are presented in parentheses. The sample includes 79,452 observations. Observations with incomplete market data are dropped. The regression achieves an $R^2 = 0.09$, $R^2_{adj} = 0.05$.} \\
*** Significant at 1\% level
** Significant at 5\% level
* Significant at 10\% level
  \end{minipage}}
\end{tabular}
\label{tab:historical_min_max}
\end{table}


==> Tables/consensus/old/mult_postsers_app_old.tex <==
\begin{table}[ht!]
\centering
\caption{Peer Influence: Multiple Posters -- Full Regression Estimates}
\begin{tabular}{ll@{\hskip 0.4in}c@{\hskip 0.4in}c@{\hskip 0.4in}c}
\toprule \toprule
 && \multicolumn{3}{c}{\textit{Dependent Variable -- $\phi_{i,j,t}$}}\\
 && Reduced Form & Full Second Stage & Random Peers \\
 && (1) & (2) & (3) \\ [2ex]
\toprule
%Intercept              &  -2.22 (0.54) *** \\
\multirow{9}{*}{\rotatebox{90}{\textit{Independent Variables}}}
& $\phi_{i,j,t-1}$            &   0.16 (0.01) ***  &   0.17 (0.01) *** &   0.16 (0.01) ***\\
& $\Bar{\phi}_{-i,j,(t-1,t)}$ &   0.11 (0.02) *** &    0.16 (0.06) ** &   -0.01 (0.02)\\
& $R_{j,t}$                   &   0.84 (0.16) *** &   0.93 (0.24) *** &   0.86 (0.16) ***\\
& $\Bar{R}_{j,t}$             &      0.46 (0.62) &      0.51 (0.71) &      0.55 (0.66) \\
& $\sigma(R_{j,t})$           &      0.18 (0.42) &     0.11 (0.67)  &      0.14 (0.45)\\
& $min_{j,t}$                 &   0.75 (0.21) *** &    0.80 (0.31) ** &   0.76 (0.21) *** \\
& $max_{j,t}$                 &    0.39 (0.18) **  &    0.59 (0.32) * &    0.41 (0.18) **\\
& $(max-min)_{j,t}$           &   -0.35 (0.17) **  &    -0.20 (0.22) &   -0.35 (0.17) * \\
&Ticker Fixed Effects & X & X & X \\
\toprule
& No. Observations: & 11,296 & 8,505 & 11,347\\
& $R^2$: & 0.12 & 0.07 & 0.11\\
& $R^2_{adj}$: & 0.07 & 0.05 & 0.07\\
\bottomrule
\end{tabular} \\
\bigskip
\begin{tabular}{cccc}
\multicolumn{4}{l}{%
  \begin{minipage}{16cm}%
    \footnotesize{ \textit{Notes}: The dependent variable is individual investor sentiment about an asset, scaled continuously between $(-\infty, \infty)$. We estimate it using the individual's previously expressed sentiment about the same asset ($\phi_{i,j,t-1}$) and a set of market control variables ($R_{j,t},\Bar{R}_{j,t},\sigma(R_{j,t}),min_{j,t},max_{j,t},(max-min)_{j,t}$). The sentiment of peers ($\Bar{\phi}_{-i,j,(t-1,t)}$) is estimated in several ways. In Column (1), we use observed, average sentiment of peers between an author's two posts. In Column (2), we estimate the sentiment of peers using an IV. In Column (3), we select a random cohort to estimate peer sentiment. Robust standard errors, clustered at the ticker level, are presented in parentheses. Observations with incomplete market data are dropped.\\
*** Significant at 1\% level
** Significant at 5\% level
* Significant at 10\% level}
  \end{minipage}}
\end{tabular}
\label{tab:consensus_full_reg}
\end{table}


==> Tables/consensus/old/network_reg_app_old.tex <==
\begin{table}[ht!]
\centering
\caption{Peer Influence: Quantifying Peer Influence -- Network Regressions}
\begin{tabular}{ll@{\hskip 0.4in}c@{\hskip 0.4in}c@{\hskip 0.4in}c}
\toprule \toprule
 && \multicolumn{3}{c}{\textit{Dependent Variable -- $\phi_{i,j,t}$}}\\
 && Reduced Form & Full Second Stage & Random Network \\
 && (1) & (2) & (3) \\ [2ex]
\toprule
\multirow{11}{*}{\rotatebox{90}{\textit{Independent Variables}}}
& $\phi_{i,j,t-1}^{-1}$            &   -0.35 (0.05) *** & -0.35 (0.05) *** &  -0.36 (0.05) ***\\
& $\phi_{i,j,t-1}^{0}$            &   0.03 (0.03) & 0.03 (0.03) &      0.03 (0.03)\\
& $\phi_{i,j,t-1}^{+1}$            &   0.22 (0.03) *** &   0.22 (0.03) *** &   0.22 (0.03) ***\\
& $\Bar{\phi}_{-i,j,t-1}$ &   0.07 (0.01) *** &   0.34 (0.07) *** & 0.02 (0.01)\\
& $R_{j,t}$                   &   0.72 (0.14) *** &   0.73 (0.14) *** &   0.74 (0.14) ***\\
& $\Bar{R}_{j,t}$             &      0.56 (0.52)  &      0.57 (0.52) &      0.64 (0.54)\\
& $\sigma(R_{j,t})$           &      -0.80 (0.50)  &     -0.76 (0.51) &     -0.80 (0.51)\\
& $min_{j,t}$                 &   0.94 (0.19) *** &   0.95 (0.20) *** &   0.95 (0.19) ***\\
& $max_{j,t}$                 &    0.56 (0.17) *** &   0.59 (0.17) *** &   0.56 (0.17) ***\\
& $(max-min)_{j,t}$           &   -0.39 (0.13) *** &  -0.36 (0.13) *** &  -0.39 (0.13) ***\\
&Ticker Fixed Effects & X & X & X\\
\toprule
& No. Observations: & 19,893 & 19,620 & 19,879\\
& $R^2$: & 0.08 & 0.08 & 0.08\\
& $R^2_{adj}$: & 0.05 & 0.05 & 0.05\\
\bottomrule
\end{tabular} \\
\bigskip
\begin{tabular}{cccc}
\multicolumn{4}{l}{%
  \begin{minipage}{16cm}%
    \footnotesize{ \textit{Notes}: The dependent variable is individual investor sentiment about an asset, scaled continuously between $(-\infty, \infty)$. We estimate it using the individual's previously expressed sentiment about the same asset ($\phi_{i,j,t-1}$) as a categorical variable, with the author not having posted previously ($\phi_{i,j,t-1}^{NA}$) as the baseline. We control for a set of market control variables ($R_{j,t},\Bar{R}_{j,t},\sigma(R_{j,t}),min_{j,t},max_{j,t},(max-min)_{j,t}$). The sentiment of posts that the author commented on previously ($\Bar{\phi}_{-i,j,t-1}$) is estimated several ways. In column (1), we present the estimate using the sentiment of posts the author previously commented on. In column (2), we use an IV to predict the sentiment of posts the author comments on. In column (3), we randomly rewire the network, connecting the author to a random set of posts about the same ticker. Robust standard errors, clustered at the ticker level, are presented in parentheses. Observations with incomplete market data are dropped.\\
*** Significant at 1\% level
** Significant at 5\% level
* Significant at 10\% level}
  \end{minipage}}
\end{tabular}
\label{tab:reg_network}
\end{table}

==> Tables/leontieff_sentiment_spillovers.tex <==
\begin{table}[ht] 
\begin{center}
    

\caption{WSB Sentiment Spillovers from the Leontieff Inverse} 
\label{tab:leontieff_sentiment_spillovers}
    \begin{tabular}{@{\extracolsep{5pt}}lcccc} 
    \hline \\[-1.8ex] 
    & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
    \cline{2-5} 
    \\[-1.8ex] & $\phi_i = -1$ & $\phi_i = +1$ & $\phi_i = -1$ & $\phi_i = +1$ \\ 
    & (1) & (2) & (3) & (4)\\ 
    \hline \\[-1.8ex] 
    
    % $R^e$ & $-$.47$^{***}$ (.07) & .01 (.03) & $-$.47$^{***}$ (.07) & .01 (.03) \\ 
    % $\widetilde{R^e}$ & $-$.18$^{***}$ (.04) & .04$^{**}$ (.02) & $-$.18$^{***}$ (.04) & .04$^{**}$ (.02) \\ 
    % $\sigma$ & $-$1.01$^{***}$ (.17) & $-$1.01$^{***}$ (.11) & $-$1.01$^{***}$ (.17) & $-$1.01$^{***}$ (.11) \\ 
    % $\phi^+_{-1}$ & $-$.48$^{***}$ (.04) & .54$^{***}$ (.03) & $-$.48$^{***}$ (.04) & .55$^{***}$ (.03) \\ 
    % $\phi^0_{-1}$ & $-$.88$^{***}$ (.04) & $-$.41$^{***}$ (.03) & $-$.87$^{***}$ (.04) & $-$.40$^{***}$ (.03) \\ 
    % $\phi^-_{-1}$ & .89$^{***}$ (.05) & $-$.21$^{***}$ (.05) & .90$^{***}$ (.05) & $-$.20$^{***}$ (.05) \\ 
    % $\phi^{\text{NA}}_{-1}$ & $-$.23$^{***}$ (.02) & .03$^{*}$ (.02) & $-$.24$^{***}$ (.02) & .01 (.02) \\ 
    $(\boldsymbol{I}-\boldsymbol{W})^{-1} \boldsymbol{\phi^+}$ & $-$.13$^{***}$ (.04) & .11$^{***}$ (.03) & $-$.08 (.07) & .08$^{*}$ (.05) \\ 
    $(\boldsymbol{I}-\boldsymbol{W})^{-1} \boldsymbol{\phi^0}$ & $-$.22$^{***}$ (.04) & $-$.13$^{***}$ (.03) & $-$.23$^{***}$ (.08) & $-$.14$^{***}$ (.05) \\ 
    $(\boldsymbol{I}-\boldsymbol{W})^{-1} \boldsymbol{\phi^-}$ & .30$^{***}$ (.06) & $-$.10$^{*}$ (.05) & $-$.001 (.11) & $-$.24$^{***}$ (.09) \\ 
    $(\boldsymbol{I}-\boldsymbol{W})^{-1} R^e$ & $-$.07 (.17) & .10 (.08) & $-$.06 (.17) & .10 (.08) \\ 
    $(\boldsymbol{I}-\boldsymbol{W})^{-1} \widetilde{R^e}$ & $-$.05 (.04) & $-$.01 (.02) & $-$.05 (.04) & $-$.01 (.02) \\ 
    $(\boldsymbol{I}-\boldsymbol{W})^{-1} \sigma$ & 1.24$^{**}$ (.51) & .36 (.36) & 1.19$^{**}$ (.51) & .34 (.36) \\ 
    $(\boldsymbol{I}-\boldsymbol{W})^{-1} \boldsymbol{\phi^+} \times \phi^{\text{NA}}_{-1}$ &  &  & $-$.08 (.08) & .04 (.05) \\ 
    $(\boldsymbol{I}-\boldsymbol{W})^{-1} \boldsymbol{\phi^0} \times \phi^{\text{NA}}_{-1}$ &  &  & .01 (.09) & .01 (.06) \\ 
    $(\boldsymbol{I}-\boldsymbol{W})^{-1} \boldsymbol{\phi^-} \times \phi^{\text{NA}}_{-1}$ &  &  & .43$^{***}$ (.13) & .21$^{**}$ (.11) \\ 
    $m$ & $-$.70$^{***}$ (.02) & $-$.04$^{***}$ (.02) & $-$.69$^{***}$ (.02) & $-$.03$^{*}$ (.02) \\ 
    
    \hline
    AIC & \multicolumn{2}{c}{169,963.5} & \multicolumn{2}{c}{169,961.3} \\
    McFadden's R\textsuperscript{2} & \multicolumn{2}{c}{.01} & \multicolumn{2}{c}{.01} \\
    N & \multicolumn{2}{c}{84,949} & \multicolumn{2}{c}{84,949} \\
    \hline 
     & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
    \end{tabular} 
\end{center}

\footnotesize{\textit{Notes:} This table presents estimated log-odds coefficients for two multinomial logit models on the expressed sentiment in WSB submissions, using different network variables to model bullish/bearish sentiment formation from Table \ref{tab:adjacent_sentiment_spillovers}. Odd columns estimate the log-odds ratio of submission $i$'s sentiment being bearish, $\phi_i = -1$. Similarly, even columns estimate the ratio of submission $i$'s sentiment being bullish, $\phi_i = +1$. Neutral submissions serve as the benchmark. The coefficients for the baseline variables, which include the excess daily return, excess weakly return, volatility, and old sentiments by the author of the submission, are not documented here, since they do not change meaningfully from Table \ref{tab:adjacent_sentiment_spillovers}. }
\end{table} 


==> Tables/market_impact_return.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Apr 15, 2021 - 22:21:31
\begin{table}[ht!] 

\begin{center}
\caption{Impact of WSB Activity on Financial Markets} 
\label{tab:market_impact_return} 
  
\begin{tabular}{lccc} 

    & Pooled & Within & \multirow{2}{*}{TSLS} \\
    & OLS & Ticker \& Week &  \\
    
    \multicolumn{4}{l}{\textbf{Dependent Variable:} $Y_{i,t} = R^e_{i,t}$} \\
    \hline 
    $\Delta A_{i,t}$ & 0.0001$^{*}$ (0.0000) & 0.0001$^{*}$ (0.0000) & $-$0.0001$^{**}$ (0.0000) \\
    Constant & 0.001$^{***}$ (0.0001) & $-$0.001$^{***}$ (0.0001) & $-$0.001$^{***}$ (0.0001) \\ 
    \hline 
    N & 116,326 & 116,326 & 115,983 \\ 
    R$^{2}$ & 0.0003 & 0.0003 & 0.0001 \\ 
    J-statistic & -- & -- & 0.00 \\
    \\[-1.8ex] 

    \multicolumn{4}{l}{\textbf{Dependent Variable:} $Y_{i,t} = \sigma_{i,t}$} \\
    \hline 
    $\Delta A_{i,t}$ & 0.001$^{***}$ (0.0001) & 0.0005$^{***}$ (0.0001) & 0.0002$^{***}$ (0.0001) \\ 
    Constant & 0.02$^{***}$ (0.0001) & $-$0.02$^{***}$ (0.0001) & $-$0.02$^{***}$ (0.0001) \\ 
    \hline 
    N & 116,326 & 116,326 & 115,983 \\ 
    R$^{2}$ & 0.01 & 0.01 & 0.0003 \\
    J-statistic & -- & -- & 0.00 \\
    \\[-1.8ex] 
    
    \multicolumn{4}{l}{\textbf{Dependent Variable:} $Y_{i,t} = v_{i,t}$} \\
    \hline 
     $\Delta A_{i,t}$ & 0.14$^{***}$ (0.01) & 0.08$^{***}$ (0.01)  & 0.09$^{***}$ (0.01) \\ 
      Constant & 0.38$^{***}$ (0.01) & $-$0.40$^{***}$ (0.01) & $-$0.40$^{***}$ (0.01) \\ 
     \hline 
    N & 116,326 & 116,326 & 115,983 \\ 
    R$^{2}$ & 0.14 & 0.23 & 0.12 \\ 
    J-statistic & -- & -- & 0.93 \\
    \hline
    
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{center} 

\footnotesize{\textit{Notes:} This table presents coefficients of three linear models for new authors on WSB discussing asset $i$ in calendar week $t$. Robust standard errors, using the method of \citet{mackinnon1985some}, are reported in parentheses. The three models are fitted to data on three stock market variables, namely excess returns $R^e_{i,t}$, volatility in excess returns $\sigma_{i,t}$, and nominal trading volumes, $v_{i,t}$, in billions of USD. The first column is an Ordinary Least Squares (OLS) regression, with the number of new unique authors, $\Delta A_{i,t}$, as the independent variable. The second column estimates an OLS regression on the within-week and within-ticker fluctuation in all dependent an independent variables. This is identical to adding week and ticker fixed effects. The final column implements a Two Stage Least Squares procedure, where the instruments for new authors are the stock of authors in the previous period, $A_{i,t-1}$, and average excess returns in the previous week, $R^e_{i,t-1}$. All variables, including instruments, remain de-meaned. The J-statistic is calculated as two times the F-statistic from a regression with residuals from the TSLS as the dependent variable, and the instruments as independent variables.}
\end{table} 


==> Tables/market_impact_simple.tex <==
\begin{table}[ht!]
\centering
\caption{Evidence of Market Impact: WSB Activity vs. Returns, Volatility and Trading Volumes}
\label{tab:market_impact_2sls}
\begin{tabular}{lccc}
\toprule \toprule
 \multicolumn{4}{l}{\textbf{Reduced Form}: market activity vs. WSB activity} \\[1ex]
&  \multicolumn{3}{c}{\textit{Dependent Variables}}  \\
\\[-1.8ex] & $R^e_{i,t}$ & $\sigma_{i,t}$ & $Q_{i,t}$ \\ 
 & (1) & (2) & (3) \\ 
 $\Delta A_{i,t}$ & 0.0001 $^{*}$ (0.0000) & 0.001$^{***}$ (0.0001) & 0.13$^{***}$ (0.01)\\ \\[-1.8ex]
  $\phi_{i,t-1}$ & $-$0.002$^{**}$ (0.001) & 0.01$^{***}$ (0.002) & 0.60$^{***}$ (0.12) \\ \\[-1.8ex]
 $\alpha$ & 0.001$^{***}$ (0.0001)& 0.03$^{***}$ (0.0001)& 0.36$^{***}$ (0.01)\\ 
\cline{1-4}
\small{R$^{2}$} & \small{0.0004}  & \small{0.01}  & \small{0.22} \\ 
\small{Adjusted R$^{2}$}& \small{0.0003} & \small{0.01}  & \small{0.22}  \\ 
\toprule
 \multicolumn{4}{l}{\textbf{First Stage IV}: predicting future WSB activity} \\[1ex]
&  \multicolumn{3}{c}{\textit{Independent Variables}}  \\
&    $min_{j,t}$ &     $max_{j,t}$ & $(max-min)_{j,t}$ \\ \cline{2-4}
Investor Sentiment $(\phi_{i,j,t})$ & 0.61 (0.15) *** & 0.32 (0.07) *** &  -0.29 (0.08) ***  \\
\small{Observations: 79,246} &&& \\[2ex]
\toprule
 \multicolumn{4}{l}{\textbf{IV}: predicting market activity} \\[1ex]
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & $R^e_{i,t}$ & $\sigma_{i,t}$ & $Q_{i,t}$ \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 $\Delta \widehat{A}_{i,t}$ & $-$0.0001$^{**}$ (0.0000) & 0.0001$^{***}$ (0.0000) & 0.09$^{***}$ (0.01) \\ 
 $\phi_{i,t-1}$ & $-$0.002 (0.001) & 0.01$^{***}$ (0.001) & 0.12$^{**}$ (0.05) \\ 
 $\alpha$ & $-$0.001$^{***}$ (0.0001) & $-$0.03$^{***}$ (0.0001) & $-$0.41$^{***}$ (0.01) \\ 
\hline \\[-1.8ex] 
FS F-statistic & 28.93 & 28.93 & 28.93 \\ 
J-statistic & 0.002 & 88.702 & 0.115 \\ 
%Observations & 64,698 & 64,698 & 64,698 \\ 
R$^{2}$ & $-$0.001 & 0.005 & 0.29 \\ 
Adjusted R$^{2}$ & $-$0.001 & 0.005 & 0.29 \\ 
\bottomrule
\end{tabular} \\
\bigskip
\begin{tabular}{cccc}
\multicolumn{4}{l}{%
  \begin{minipage}{17cm}%
    \footnotesize{ \textit{Notes}: The first stage is estimated using all submission data from WSB. The second stage is estimated using the average predicted sentiment of peers between an author's posts about the same asset. Ticker-level dummies, asset return and volatility controls, and the intercept are included in the second stage but not shown. Robust standard errors, clustered at the ticker level, are presented in parentheses. Observations with incomplete market data are dropped. The first stage regression achieves an $R^2 = 0.001$, $R^2_{adj} = 0.001$. The second stage has $R^2 = 0.1$, $R^2_{adj} = 0.047$.\\
*** Significant at 1\% level
** Significant at 5\% level
* Significant at 10\% level}
  \end{minipage}}
\end{tabular}
\label{tab:reg_market_2sls}
\end{table}




==> Tables/market_impact_tsls.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, May 04, 2021 - 10:22:57
\begin{table}[ht] 
\begin{center}
  \caption{2SLS Estimate for the impact of WSB Activity on Assets} 
  \label{tab:market_impact_tsls} 
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & $R^e_{i,t}$ & $\sigma_{i,t}$ & $Q_{i,t}$ \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 $\Delta \widehat{A}_{i,t}$ & $-$0.0001$^{**}$ (0.0000) & 0.0001$^{***}$ (0.0000) & 0.09$^{***}$ (0.01) \\ 
 $\phi_{i,t-1}$ & $-$0.002 (0.001) & 0.01$^{***}$ (0.001) & 0.12$^{**}$ (0.05) \\ 
 $\alpha$ & $-$0.001$^{***}$ (0.0001) & $-$0.03$^{***}$ (0.0001) & $-$0.41$^{***}$ (0.01) \\ 
\hline \\[-1.8ex] 
FS F-statistic & 28.93 & 28.93 & 28.93 \\ 
J-statistic & 0.002 & 88.702 & 0.115 \\ 
%Observations & 64,698 & 64,698 & 64,698 \\ 
R$^{2}$ & $-$0.001 & 0.005 & 0.29 \\ 
Adjusted R$^{2}$ & $-$0.001 & 0.005 & 0.29 \\ 
\hline 
\hline
 & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{center}

\footnotesize{\textit{Notes:} This table presents coefficients of our 2SLS model in Eqs. \ref{eq:ols_caus}-\ref{eq:first_stage} for the predicted new authors on WSB discussing asset $i$ in calendar week $t$, $\Delta \widehat{A}_{i,t}$, and the average sentiment expressed about asset $i$ in the previous week $t-1$, $\phi_{i,t-1}$, fitted to data on three stock market variables: excess returns $R^e_{i,t}$, volatility in excess returns $\sigma_{i,t}$, and nominal trading volumes, $Q_{i,t}$. Each regression is estimated on 64,698 observations. We use the number of authors who commented in the preceding three weeks, as well as average price returns in previous week, as instrumental variables in predicting the number of new authors in the current week. The within-transformation is applied to all variables, with respect to tickers $i$ and weeks $t$. FS F-statistic denotes the F-statistic on the first-stage regression, testing whether the coefficients on the instrumental variables are simultaneously equal to zero. The J-statistic is computed in the fashion of Sargan-Hansen.}
\end{table} 


==> Tables/returns.tex <==
\begin{table}[ht!]
\centering
\caption{Hype Investor Returns}
\label{tab:market_impact_returns}
\begin{tabular}{lccccc}
\toprule \toprule
 \multicolumn{6}{l}{\textbf{Cumulative Returns on WSB Advice: expressed in (\%)}} \\[1ex]
&  \multicolumn{5}{c}{\textit{Return Time Horizon}}  \\
\\[-1.8ex] & Next Day & 3 Days & 1 Week & 4 Weeks & 12 Weeks\\ 
 & (1) & (2) & (3) & (4) & (5)\\ 
\textit{Overall Return} &        -0.13 &      -0.25 &          -0.35 & -0.45 & -1.02 \\
\textit{Short Only Return} & -0.02 &        0.08 &      0.04 &          -0.60 & -3.47 \\
\hline
\textit{Most Popular Tickers} &  &  &  & & \\
\hspace{10mm} Top 10 & 0.07 & 0.34 & 0.47 & 1.48 & 5.42 \\
\hspace{10mm} Top 20 & -0.06 & 0.14 & 0.25 & 0.78 & 3.19 \\
\hspace{10mm} Top 50 & -0.05 & 0.10 & 0.20 & 0.51 & 1.61 \\
\hspace{10mm} Top 500 & -0.01 & -0.05 & -0.12 & -0.43 & -0.40 \\
\hline
\textit{SPY Portfolio} & 0.04 & 0.11 & 0.20 & 0.82 & 2.54\\  
\bottomrule
\end{tabular} \\
\bigskip
\begin{tabular}{cccc}
\multicolumn{4}{l}{%
  \begin{minipage}{17cm}%
    \footnotesize{ \textit{Notes}: We present the cumulative returns, in percentage points, for investing \$1 each day that WSB is active into a WSB portfolio, constructed using the extracted tickers and sentiments from posts -- the portfolio construction is detailed in Appendix \ref{app:market_impact}. We also consider a portfolio where we invest only in bearish posts - \textit{Short Only Return}. We also construct the portfolio looking only at posts in the most popular tickers on WSB. We compare this to investing the same \$1 into $SPY$.}
  \end{minipage}}
\end{tabular}
\end{table}




==> Tables/sentiment_regression.tex <==
\begingroup
\renewcommand{\arraystretch}{0.85}
\begin{table}[htbp]

\begin{center}
    \caption{WSB Sentiments and Asset Price Movements} 
    \label{tab:sentiment_regression_table} 
        \begin{tabular}{@{\extracolsep{5pt}}lccc} 
        \\[-1.8ex]\hline 
        \hline \\[-1.8ex] 
         & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
        \cline{2-4} 
        \\[-1.8ex] & $R_{i,t}^e$ & $\log (V_{i,t})$ & $\log(P_{i,t}^H/P_{i,t}^L)$ \\ 
        \\[-1.8ex] & (1) & (2) & (3)\\ 
        \hline \\[-1.8ex] 
        
            $\Phi_{i,t}^+$ & 0.004 (0.0001) & 0.15 (0.004) & 0.01 (0.0001) \\ 
            $\Phi_{i,t}^0$ & 0.002 (0.0001) & 0.09 (0.003) & 0.01 (0.0001) \\ 
            $\Phi_{i,t}^-$ & $-$0.01 (0.0002) & $-$0.13 (0.01) & $-$0.01 (0.0002) \\ \\[-1.8ex] 
            \hline  \\[-1.8ex]
            Within-ticker & Yes & Yes & Yes \\
            Within-day & Yes & Yes & Yes \\
            N & 14.4m & 14.4m & 14.4m \\
            Adjusted R$^{2}$ & .0002 & .0005 & .001 \\
            \hline 
        \end{tabular}
\end{center}

\footnotesize{\textit{Notes:} This table presents OLS estimators for the correlation between aggregated daily sentiments on WSB, $\Phi_{i,t}^s$, and three stock market indicators as dependent variables. All variables are `within'-transformed to denote their deviations from cross-sectional and temporal means. Subscript $i$ denotes the asset, and $t$ the trading day. Superscripts $+$, $0$ and $-$ denote bullish, neutral and bearish sentiments, respectively. Corresponding standard errors are given in parentheses. Column (1) uses daily returns, calculated as the ratio of subsequent closing prices for asset $i$ at times $t$ and $t-1$, as recorded in CRSP, minus the risk free rate, as reported in K. French's data library. Columns (2) and (3) regress the variation in sentiment within asset $i$ and time $t$ on the within asset and time variations in log of trading volume. The same is done in column (3) for the log-difference in daily intra-day high and low prices for asset $i$.}
\end{table}
\endgroup

==> Tables/submission_time_series_regression.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Mon, Apr 12, 2021 - 10:20:53
\begin{table}[ht]
    
\begin{center}
\caption{Time Dynamics of Assets Discussed on WSB} 
\label{tab:submission_time_series_regression} 
  
    \begin{tabular}{@{\extracolsep{5pt}}lccc} 
    \\[-1.8ex]\hline 
    \hline \\[-1.8ex] 
    
    & \multicolumn{3}{c}{\textit{Dependent variable:} $\Delta A_{i,t}$} \\ 
    \cline{2-4} \\[-1.8ex]
    & (1) & (2) & (3)\\ 
    \hline \\[-1.8ex] 
    
    $A_{i,t-1}$ & 0.40$^{***}$ (0.002) & 0.40$^{***}$ (0.002) & 0.38$^{***}$ (0.002) \\ 
    $\sum_{j=1}^{3} A_{i,t-j}$ & $-$0.06$^{***}$ (0.001) & $-$0.06$^{***}$ (0.001) & $-$0.06$^{***}$ (0.001) \\ 
    $R^e_{i,t}$ &  &  & $-$1.07$^{**}$ (0.47) \\ 
    $\sigma_{i,t}$ &  &  & 11.64$^{***}$ (0.34) \\ 
    $Q_{i,t}$ &  &  & 0.48$^{***}$ (0.01) \\ 
    $\alpha$ & 0.15$^{***}$ (0.01) & $-$0.002 (0.01) & $-$0.01 (0.01) \\ 
    \hline \\[-1.8ex] 
    
    Model & Pooled & Within-week & Within-week \\
    N & 118,024 & 118,024 & 116,326 \\ 
    Adjusted R$^{2}$ & 0.49 & 0.48 & 0.51 \\ 
    \hline 
    \hline 
    \textit{ }  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
    \end{tabular} 
\end{center}
\footnotesize{\textit{Notes:} This table presents coefficients for an OLS model estimating the number of new users, $\Delta A_{i,t}$, discussing a ticker on WSB from the set of independent variables in Eq. \ref{eq:new_user_ols}}: $A_{i,t-1}$ is the number of unique authors who posted a submission on ticker $i$ in weeks $t-1$ to $t-3$, and $\sum_{j=1}^{3} A_{i,t-j}$ is the cumulative count of unique authors. Column (1) estimates the OLS coefficients by pooling all the available data, and column (2) subtracts the cross-sectional mean in a given week from each variable, to control for unobserved time heterogeneity (as denoted by `Within-week' under the Model label). In particular, we may be concerned with WSB boasting a larger following in recent years. In column (3), we include controls for the average price return, $R^e_{i,t}$, price return standard deviation, $\sigma_{i,t}$, and average dollar trading volumes, $Q_{i,t}$, for asset $i$ in week $t$. Details on the construction of financial variables are provided in Appendix \ref{app:data_appendix}.
\end{table} 

==> Tables/topic_model1.tex <==
    \begin{table}[!htbp]
    {
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    \textbf{Topic Title} & \textbf{Top Words} & \textbf{Topic Prevalence (\%)} \\
    \hline
Robinhood Trading Limits & \multicolumn{1}{m{8cm}|}{robinhood, gme, account, nkla, margin, order, app, limit, broker, orders} & 1.8 \\
 \hline 
International Trade & \multicolumn{1}{m{8cm}|}{expected, yr, china, usd, europe, japan, pmi, manufacturing, korea, data} & 0.8 \\
 \hline 
Retail Sales + Amazon & \multicolumn{1}{m{8cm}|}{sales, amazon, home, stores, business, online, companies, food, store, retail} & 3.0 \\
 \hline 
Top Stock Picks / Positions & \multicolumn{1}{m{8cm}|}{tsla, news, sold, aapl, weeks, holding, hold, amd, months, dip} & 11.6 \\
 \hline 
Other & \multicolumn{1}{m{8cm}|}{comments, daily, best, moves, spy, weekend, fo, fn, fm, fp} & 1.1 \\
 \hline 
Other & \multicolumn{1}{m{8cm}|}{mentions, vote, log, wsbvotebot, submission, posts, check, reverse, mention, great} & 0.2 \\
 \hline 
Electric Cars & \multicolumn{1}{m{8cm}|}{tsla, energy, car, ev, cars, nio, electric, battery, elon, space} & 2.3 \\
 \hline 
Revenues, Earnings, Ratings & \multicolumn{1}{m{8cm}|}{revs, beats, tgt, line, eps, neutral, downgraded, initiated, fy, reports} & 0.9 \\
 \hline 
FDA / Pharma & \multicolumn{1}{m{8cm}|}{drug, fda, phase, patients, vaccine, trial, treatment, results, clinical, covid} & 2.9 \\
 \hline 
Revenues, Earnings, Ratings & \multicolumn{1}{m{8cm}|}{revenue, million, growth, quarter, share, sales, billion, net, expected, eps} & 4.0 \\
 \hline 
China Trade Deal & \multicolumn{1}{m{8cm}|}{trump, china, said, president, deal, bill, house, election, chinese, news} & 3.1 \\
 \hline 
Social Media Stocks & \multicolumn{1}{m{8cm}|}{fb, game, snap, aapl, disney, games, video, google, users, netflix} & 2.7 \\
 \hline 
GME Discussion & \multicolumn{1}{m{8cm}|}{companies, gme, investors, world, years, believe, hedge, actually, value, funds} & 7.3 \\
 \hline 
Financial News & \multicolumn{1}{m{8cm}|}{data, information, news, financial, report, based, find, sec, research, investors} & 4.3 \\
 \hline 
Personal Discussions & \multicolumn{1}{m{8cm}|}{life, wife, ass, little, said, spy, getting, old, red, went} & 7.6 \\
 \hline 
Weed Stocks & \multicolumn{1}{m{8cm}|}{million, share, capital, ceo, cannabis, ipo, public, management, merger, billion} & 2.1 \\
 \hline 
     \end{tabular}
    \caption{\textbf{Topics Extracted from BTM Model (1)}}
    \label{table::btm_topics1}}
    \end{table}

==> Tables/topic_model2.tex <==
    \begin{table}[!htbp]
    \begin{center}
    \begin{tabular}{|c|c|c|}
    \hline
    \textbf{Topic Title} & \textbf{Top Words} & \textbf{Topic Prevalence (\%)} \\
    \hline
Software Tech Stocks & \multicolumn{1}{m{8cm}|}{amd, aapl, intc, companies, data, cloud, software, technology, services, tech} & 3.4 \\
 \hline 
Earnings Release & \multicolumn{1}{m{8cm}|}{release, estimates, consensus, share, revenue, move, open, beat, average, interest} & 1.0 \\
 \hline 
Natural Resources & \multicolumn{1}{m{8cm}|}{oil, gold, prices, silver, gas, futures, crude, production, demand, companies} & 1.8 \\
 \hline 
FED / Rates & \multicolumn{1}{m{8cm}|}{fed, rates, rate, economy, markets, economic, said, interest, growth, inflation} & 6.0 \\
 \hline 
Other Tech Stocks & \multicolumn{1}{m{8cm}|}{tsla, pltr, elon, musk, mods, ban, gme, retards, gains, autists} & 2.0 \\
 \hline 
COVID / China & \multicolumn{1}{m{8cm}|}{virus, covid, cases, coronavirus, china, world, weeks, corona, states, news} & 4.8 \\
 \hline 
Other & \multicolumn{1}{m{8cm}|}{spy, bear, gay, text, bears, bull, gang, msft, words, stonks} & 1.7 \\
 \hline 
Debt / Loans & \multicolumn{1}{m{8cm}|}{debt, cash, pay, credit, loans, loan, million, interest, billion, bank} & 3.4 \\
 \hline 
Other & \multicolumn{1}{m{8cm}|}{usd, bln, exp, revenue, newswires, eps, co, share, symbol, live} & 1.4 \\
 \hline 
Other & \multicolumn{1}{m{8cm}|}{spy, chart, close, index, month, performance, major, past, futures, sectors} & 1.3 \\
 \hline 
Account Help & \multicolumn{1}{m{8cm}|}{account, help, investing, best, start, robinhood, advice, work, years, please} & 7.4 \\
 \hline 
Other & \multicolumn{1}{m{8cm}|}{spy, volume, chart, support, bullish, low, trend, resistance, bearish, line} & 3.7 \\
 \hline 
Other & \multicolumn{1}{m{8cm}|}{amet, calendar, releases, wed, link, thurs, tues, fri, analyst, close} & 0.5 \\
 \hline 
Options / Risk & \multicolumn{1}{m{8cm}|}{option, spy, profit, strike, spread, risk, loss, value, selling, position} & 6.3 \\
 \hline 
     \end{tabular}
    \end{center}
    \caption{\textbf{Topics Extracted from BTM Model (2)}}
    \label{table::btm_topics2}
    \end{table}

==> Tables/variable_normalization.tex <==
\begin{table}[!ht]
\begin{center}
  \caption{Variable mean and standard deviation} 
  \label{tab:variable_norm} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\toprule \\[-1.8ex] 
\textbf{Variables} & \textbf{Mean (standard deviation)} \\ 
$r_{j,1day}$ & -0.001 (0.037) \\
$\Bar{r}_{j,5day}$ & -0.001 (0.016)\\
$\sigma^2_{j,5day}$ & 0.001 (0.011)\\
$\Bar{\Phi}_{-i,j,(t-1,t)}$ \textit{Frequent Posters} & 0.658 (0.751) \\
$\Bar{\Phi}_{-i,j,(t-1,t)}$ \textit{Commenter Network} & 0.664 (1.171) \\
IV \textit{Frequent Posters} & 0.705 (0.271) \\
IV \textit{Commenter Network} & 0.654 (0.168) \\
\bottomrule 
\end{tabular} 
\end{center}
\vspace{-0.6em}
\footnotesize{ \textit{Notes}:}

\end{table}

==> Tables/variant1_model.tex <==
\begin{table}[!ht]
\begin{center}
  \caption{Estimating the Peer Effects as $\theta$ in \cite{bordalo2021diagnostic}.} 
  \label{tab:model_variant1} 
 \def\arraystretch{1.4}
\begin{tabular}{@{\extracolsep{5pt}}lcc} 
\toprule \\[-1.8ex] 

& \multicolumn{2}{c}{\textit{Dependent variable:} Sentiment of Post: $\Phi_{i,j,t}$} \\
& Reduced Form & 2SLS \\
& (Observed Peer Sentiment) & (Predicted Peer Sentiment using IV) \\
& (1) & (2) \\
\cline{2-3} \\[-1.8ex] 
$\Bar{\Phi}_{-i,j,(t-1,t)}$ &   0.11 (0.02) *** & 0.13 (0.01) ***\\
$\Phi_{i,j,t-1}$ & 0.15 (0.01) *** & 0.20 (0.05) ***\\
$r_{j,t}$ & 0.67 (0.20) *** & 0.17 (0.38) \\
$\Bar{r}_{j,t}$ & 0.61 (0.35) * & 0.75 (0.47) \\
$\sigma^2_{j,t}$ & -0.21 (0.57) & 0.58 (1.01) \\
$\mathbf{r_{j,t} \times \Bar{\Phi}_{-i,j,(t-1,t)}}$ & 0.17 (0.15) & 1.08 (0.50) ***\\
Ticker Fixed Effects & Yes & Yes \\
  \hline
    Number of obs. & 14,396 & 14,396 \\ 
    Adjusted R$^{2}$ & 0.08  &  0.08 \\
    F Statistic & 139 & 57\\ 
\bottomrule \\[-1.8ex] 
\end{tabular} 
\end{center}

\footnotesize{ \textit{Notes}: The dependent variable is individual investor sentiment about an asset expressed in a single submission, scaled continuously between $(-\infty, \infty)$. We estimate it using the individual's previously expressed sentiment about the same asset ($\Phi_{i,j,t-1}$), as well as the average sentiment of peer posts that the author is exposed two between their two posts ($\Bar{\Phi}_{-i,j,t-1}$), returns $r_{j,t}$, $\Bar{r}_{j,t}$, asset volatility $\sigma^2_{j,t}$. 

*** Significant at 1\% level ** Significant at 5\% level * Significant at 10\% level}

\end{table}
